Geometric Impedance Control on SE(3) for Robotic Manipulators

After its introduction, impedance control has been utilized as a primary control scheme for robotic manipulation tasks that involve interaction with unknown environments. While impedance control has been extensively studied, the geometric structure of SE(3) for the robotic manipulator itself and its use in formulating a robotic task has not been adequately addressed. In this paper, we propose a differential geometric approach to impedance control. Given a left-invariant error metric in SE(3), the corresponding error vectors in position and velocity are first derived. We then propose the impedance control schemes that adequately account for the geometric structure of the manipulator in SE(3) based on a left-invariant potential function. The closed-loop stabilities for the proposed control schemes are verified using Lyapunov function-based analysis. The proposed control design clearly outperformed a conventional impedance control approach when tracking challenging trajectory profiles.

==> chapters/A_combined_old.tex <==
\subsection{Comments on left perturbation for error function}
\vspace{-12pt}
Perturbation of the error function using left translation is
\begin{align*}
    \delta g_\eta = \hat{\eta}\g = \begin{bmatrix}
    \hat{\omega}R & \hat{\omega} p + v \\
    0 & 0 
    \end{bmatrix} = \begin{bmatrix}
    \delta R & \delta p \\ 0 & 0
    \end{bmatrix}
\end{align*}
The perturbation of the error function gives
\begin{align*}
    \delta \Psi(\g,\gd)&=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\delta R^T R_d\!-\!R_d^T \delta R & \ast
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T \delta \pvec
    \end{bmatrix}\\
    &= \dfrac{1}{2}\tr(\hat{\omega}R^T R_d - R_d R^T \hat{\omega}) + (\pvec - \pvecd)^T(\hat{\omega}\pvec + v)
\end{align*}
However, it does not provide insightful result when it is represented in
\begin{align*}
    \delta \Psi(\g,\gd) = e_g^{'T} V^s,
\end{align*}
where $V^s$ is the spatial velocity.
\vspace{-10pt}
\subsection{A derivation of the time-derivative of the potential energy part}
\vspace{-12pt}
The time-derivative of the potential function is
\begin{align*}
    \dfrac{dP}{dt} = \dfrac{1}{2}\tr(\dot{\psi}_k^T\psi_k) + \dfrac{1}{2}\tr(\psi_k^T \dot{\psi}_k) = \tr(\psi_k^T \dot{\psi}_k)
\end{align*}
Where,
\begin{align*}
    &\dot \psi_k = 
    \dfrac{d\psi_k}{dt} 
    % &= \begin{bmatrix}
    % \sqrt{K_o}(\hat{\omega}_d R_d^T R - R_d^TR\hat{\omega}) & m_{12}\\
    % 0 & 0 
    % \end{bmatrix} 
    = \begin{bmatrix}
    -\sqrt{K_o}R_d^T R \hat{e}_\Omega & m_{12}\\
    0 & 0
    \end{bmatrix},\mbox{with }\\
     &m_{12} = \hat{\omega}_d R_d^T \sqrt{K_t}(\pvec - \pvecd) - R_d^T \sqrt{K_t}Rv + R_d^T\sqrt{K_t}R_dv_d.
\end{align*}
Which leads to the form of
\begin{align*}
    \dfrac{dP}{dt} = \tr\left(\begin{bmatrix}
    a_{11} & \ast \\
    \ast & a_{22}
    \end{bmatrix}
    \right)
\end{align*}
where $\ast$ terms are not of interest because of the trace operator. 
\begin{align*}
    a_{11} &= (I - R^TR_d)\sqrt{K_o}^T (-\sqrt{K_o})R_d R \hat{e}_\Omega  \\
    a_{22} &= -(\pvec - \pvecd)^T\sqrt{K_t}^TR_d m_{12}
\end{align*}
Using the assumption that $K_o$ is diagonal matrix, and matrices are commutable in the trace, i.e., $\tr(AB) = \tr(BA)$,
\begin{align*}
    \tr(a_{11}) &= \tr(K_o(R_d^TR - I)\hat{e}_\Omega)\\
    &= - \tr(K_o(R_d^TR\hat{e}_\Omega)) + \tr(K_o \hat{e}_\Omega)\\
    &= -\dfrac{1}{2}\tr(K_o(R_d^T R \hat{e}_\Omega \!-\! \hat{e}_\Omega R^T R_d)) = -\dfrac{1}{2}\tr(\hat{e}_\Omega K_o \hat{e}_R)
\end{align*}
Note also that for $x = [x_1, x_2, x_3]^T$, $y = [y_1, y_2, y_3]^T$, and $\Sigma = \text{diag}([\sigma_1,\sigma_2,\sigma_3])$,
\begin{align*}
    \tr(\hat{x}\Sigma \hat{y}) = -x^T \begin{bmatrix}
    \sigma_2 +\sigma_3 & 0 & 0 \\
    0 & \sigma_1 + \sigma_3 & 0 \\
    0 & 0 & \sigma_1 + \sigma_2
    \end{bmatrix} y.
\end{align*}
Therefore, $\tr(a_{11}) = e_\Omega^T \tilde{K}_o e_R$.\\
% \begin{align*}
    % \tr(a_{11}) = e_\Omega^T \tilde{K}_o e_R.
% \end{align*}
On the other hand, $\tr(a_{12})$ can be unraveled as
\begin{align*}
    &\tr(a_{22}) = \tr\left(-(\pvec - \pvecd)^T K_t R_d \hat{\omega}_d R_d^T(\pvec - \pvecd)\right) \\
    &\; + \tr\left((\pvec - \pvecd)^T R R^T K_t Rv - (\pvec - \pvecd)^TR R^T K_t R_d v_d\right)\\
    &= \tr\left(-(\pvec - \pvecd)R R^T K_t R_d\hat{\omega}_d R_d^T(\pvec - \pvecd) \right) \\
    & \;+ \tr\left((\pvec - \pvecd)^T R K_t (v - R^TR_d v_d) \right)\\
    &= \tr\left((\pvec - \pvecd)^T R K_t (v - R^TR_d - R^TR_d \omega_d R_d^T (\pvec - \pvecd)\right)\\
    &= \tr\left(e_p^T K_t e_v\right) = e_v^T K_t e_p
\end{align*}
since $e_p^T K_t e_v$ is a scalar. 
Putting all things together,
\begin{align*}
    \dfrac{dP}{dt} = \ev^T \begin{bmatrix}
    K_t & 0 \\
    0 & \tilde{K}_o
    \end{bmatrix} \eg
\end{align*}
is shown.


==> chapters/A_derivPotEn.tex <==
The time-derivative of the potential function is
\begin{align*}
    \dfrac{dP}{dt} = \dfrac{1}{2}\tr(\dot{\psi}_k^T\psi_k) + \dfrac{1}{2}\tr(\psi_k^T \dot{\psi}_k) = \tr(\psi_k^T \dot{\psi}_k)
\end{align*}
Then,
\begin{align*}
    &\dfrac{d\psi_k}{dt} 
    % &= \begin{bmatrix}
    % \sqrt{K_o}(\hat{\omega}_d R_d^T R - R_d^TR\hat{\omega}) & m_{12}\\
    % 0 & 0 
    % \end{bmatrix} 
    = \begin{bmatrix}
    -\sqrt{K_o}R_d^T R \hat{e}_\Omega & m_{12}\\
    0 & 0
    \end{bmatrix},\\
    &m_{12} = \hat{\omega}_d R_d^T \sqrt{K_t}(\pvec - \pvecd) - R_d^T \sqrt{K_t}Rv + R_d^T\sqrt{K_t}R_dv_d.
\end{align*}
Which leads to the form of
\begin{align*}
    \dfrac{dP}{dt} = \tr\left(\begin{bmatrix}
    a_{11} & \ast \\
    \ast & a_{22}
    \end{bmatrix}
    \right)
\end{align*}
where $\ast$ terms are not interested because of trace operator. 
\begin{align*}
    a_{11} &= (I - R^TR_d)\sqrt{K_o}^T (-\sqrt{K_o})R_d R \hat{e}_\Omega  \\
    a_{22} &= -(\pvec - \pvecd)^T\sqrt{K_t}^TR_d m_{12}
\end{align*}
Using the assumption that $K_o$ is diagonal matrix, and matrices are commutable in the trace, i.e., $\tr(AB) = \tr(BA)$,
\begin{align*}
    \tr(a_{11}) &= \tr(K_o(R_d^TR - I)\hat{e}_\Omega)\\
    &= - \tr(K_o(R_d^TR\hat{e}_\Omega)) + \tr(K_o \hat{e}_\Omega)\\
    &= -\dfrac{1}{2}\tr(K_o(R_d^T R \hat{e}_\Omega - \hat{e}_\Omega R^T R_d)) = -\dfrac{1}{2}\tr(\hat{e}_\Omega K_o \hat{e}_R)
\end{align*}
Note also that for $x \in [x_1, x_2, x_3]^T$, $y \in [y_1, y_2, y_3]^T$, and $\Sigma = \text{diag}([\sigma_1,\sigma_2,\sigma_3])$,
\begin{align*}
    \tr(\hat{x}\Sigma \hat{y}) = -x^T \begin{bmatrix}
    \sigma_2 +\sigma_3 & 0 & 0 \\
    0 & \sigma_1 + \sigma_3 & 0 \\
    0 & 0 & \sigma_1 + \sigma_2
    \end{bmatrix} y.
\end{align*}
Therefore, $\tr(a_{11}) = e_\Omega^T \tilde{K}_o e_R$.\\
% \begin{align*}
    % \tr(a_{11}) = e_\Omega^T \tilde{K}_o e_R.
% \end{align*}
On the other hand, $\tr(a_{22})$ is unraveled as
\begin{align*}
    &\tr(a_{12}) = \tr\left(-(\pvec - \pvecd)^T K_t R_d \hat{\omega}_d R_d^T(\pvec - \pvecd)\right) \\
    &\; + \tr\left((\pvec - \pvecd)^T R R^T K_t Rv - (\pvec - \pvecd)^TR R^T K_t R_d v_d\right)\\
    &= \tr\left(-(\pvec - \pvecd)R R^T K_t R_d\hat{\omega}_d R_d^T(\pvec - \pvecd) \right) \\
    & \;+ \tr\left((\pvec - \pvecd)^T R K_t (v - R^TR_d v_d) \right)\\
    &= \tr\left((\pvec - \pvecd)^T R K_t (v - R^TR_d - R^TR_d \omega_d R_d^T (\pvec - \pvecd)\right)\\
    &= \tr\left(e_p^T K_t e_v\right) = e_v^T K_t e_p
\end{align*}
since $e_p^T K_t e_v$ is a scalar. 
Putting all things together,
\begin{align*}
    \dfrac{dP}{dt} = \ev^T \begin{bmatrix}
    K_t & 0 \\
    0 & \tilde{K}_o
    \end{bmatrix} \eg
\end{align*}
is shown.


==> chapters/A_left_perturbation.tex <==
Perturbation of the error function using left translation is
\begin{align*}
    \delta g_\eta = \hat{\eta}\g = \begin{bmatrix}
    \hat{\omega}R & \hat{\omega} p + v \\
    0 & 0 
    \end{bmatrix} = \begin{bmatrix}
    \delta R & \delta p \\ 0 & 0
    \end{bmatrix}
\end{align*}
The perturbation of the error function gives
\begin{align*}
    \delta \Psi(\g,\gd)&=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\delta R^T R_d\!-\!R_d^T \delta R & \ast
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T \delta \pvec
    \end{bmatrix}\\
    &= \dfrac{1}{2}\tr(\hat{\omega}R^T R_d - R_d R^T \hat{\omega}) + (\pvec - \pvecd)^T(\hat{\omega}\pvec + v)
\end{align*}
However, it does not provide insightful result when it is represented in
\begin{align*}
    \delta \Psi(\g,\gd) = e_g^{'T} V^s,
\end{align*}
where $V^s$ is the spatial velocity.

==> chapters/ch1_intro_old.tex <==
Impedance control was first proposed to solve the manipulator's end-effector positioning problem based on an operational space frame formulation \cite{hogan1985impedance, khatib1987unified}.
% The intuitive structure of the impedance control raise lots of research interests since its first proposal.
Since then, it has been the main framework for controlling the end-effector position, particularly on tasks that involve potential contact interaction with the environment, and is thereby widely utilized in robotic manipulation. 

%Impedance control also plays a fundamental role in interacting with unknown environments. 
By specifying a desired end-effector impedance relative to its body frame, it is possible to  attain safe robot interaction with its environment  and closed loop stability robustness in the execution of assembly tasks \cite{chen2013robotic, khan2010safe, ott2008passivity}. To better deal with the unknown environment, impedance control is often combined with learning algorithms; adaptive control approaches such as \cite{li2010learning, duan2018adaptive},
behavior cloning approaches including \cite{rozo2016learning, abu2018force}
and reinforcement learning approaches \cite{zhang2021learning, martin2019variable, luo2019reinforcement}.

% The implementation of the impedance control is based on the error terms.
Tracking errors in impedance control are often calculated separately as  translation and orientation errors in the spatial frame. To define the orientation error, \cite{caccavale1999six} proposed methods utilizing rotation matrices. The concept of using the geometry of $\SO$ to define orientation errors is widely employed, e.g., \cite{robosuite2020, ochoa2021impedance}. However surprisingly to date, most  schemes utilized for separating translation and orientation errors do not adequately consider the geometry of $\SE$, even though the end-effector lies in  $\SE$.
% the geometric structure of $\SE$ is not considered.

A spatial spring defined in $\SE$ was utilized in robotic applications by \cite{stramigioli2001variable} and also in the control of Unmanned Aerial Vehicles (UAV) by \cite{rashad2019energy}. The wrenches from the spatial springs and linear dampers are utilized as the control inputs. Based on a defined spatial spring, the impedance control was derived in \cite{fasse1997spatial} in the spatial frame. Although the manifold structure of $\SE$ is considered in these works,  results involving time-varying trajectories and a  stability analysis were not provided. 

% \JS{This should be the punchline, but it is a little bit weird.} 
Thus, to the best of our knowledge, the intrinsic manifold and geometrical structure of impedance control from the control perspective has not yet been rigorously examined. 
For example, in general,  desired and current Cartesian velocities are directly compared even though they are not in the same tangent spaces of the $\SE$ manifold. 
%
% \JS{In addition, the error metrics, or known as potential functions, defined in $\SE$ for general impedance control approaches are left-invariant metrics - which will be elaborated in Section.~\ref{Sec:3}.(This is controversial)} 
%
Additionally, since there is no bi-invariant error metric in $\SE$ \cite{park1995distance, bullo1995proportional}, the position error vectors need to  defined so they are consistent with the error metric that has been selected. 
% Additionally in $\SE$, depending on which error metric chosen, one should first check if it is left or right invariant, and the errors in position should be selected accordingly, since there is no bi-invariant metric in $\SE$ \cite{park1995distance, bullo1995proportional}.
% In $\SO$, using spatial frame or body frame makes no differences if the metric is bi-invariant, but that does not holds true when it comes to $\SE$ \cite{park1995distance, bullo1995proportional}.
% -- there is even no bi-invariant metric in $\SE$.
% \JS{Thus, the error metrics, or known as potential functions of springs, defined in $\SE$ should be first checked if it is left or right invariant, and the errors in position should be selected accordingly.}
For example, utilizing spatial frame-based error vectors for left-invariant metrics is inconsistent with its geometry. The performance can be increased when  error vectors are appropriately defined.
% \JS{By using the error in position and velocity not lying on the tangent space of the manifold, the resulting control input also does not lie on the cotangent space of the manifold, i.e., the control torque does not have appropriate direction. }
% \JS{Therefore, the control input of traditional impedance control is energy inefficient. MAY NOT BE TRUE}

In this paper, we revisit  impedance control for robotic manipulators in the context of differential geometry. By defining  position and velocity  errors in the end-effector body frame that are  intrinsically consistent with its geometry, we propose a novel control law for impedance control. Its is shown with a numerical simulation example, that our proposed control scheme outperforms  conventional impedance control approaches in trajectory tracking. This paper can be considered as an extension of \cite{lee2010geometric} from $\SO$ to $\SE$ and from UAVs to robotic manipulators. In addition, we suggest matrix impedance gains as compared to scalar gains, which is important in the framework of the variable impedance control. We emphasize that having correct error vectors will be critical to learning the required variable impedance control gains, in many learning assembly operations, since this will minimize the detrimental effects during learning cause by erroneous manipulator behavior due to inconsistent error tracking.
% \AR{Maybe: We assume that therefore a potential to increase energy efficiency exists compared to the traditional impedence control.}

The paper is organized as follows:
%
Section.~\ref{Sec:2}, presents a brief review of Lie groups in $\SO$ and $\SE$ and their their respective $\so$ and $\se$ algebras, as well a brief review of its use in forward kinematics, and  manipulator dynamics.
%
In Section~\ref{Sec:3}, the error function in $\SE$ proposed in this paper and its corresponding error vectors are derived. Using the geometrically consistent error vector, we propose a novel control law for impedance control. The derivation for the proposed approach and the stability analysis of the closed-loop system are provided as well. 
%
Section~\ref{Sec:4} shows the simulation results of the proposed approach. The benchmark results are also presented in comparison to the conventional impedance controller.
%
Finally, the concluding remarks and future works are discussed in Section~\ref{Sec:5}.

==> chapters/ch2_manDyn_old.tex <==
\subsection{Lie group and Lie algebra}
In this subsection, we briefly review the contents of group structure and its geometry.
%
For the detailed description regarding Lie group \& Lie algebra and their applications to robotics, the eader is referred to \cite{murray2017mathematical} and \cite{lynch2017modern}.
%
The configuration of the robotic manipulator's end-effector is defined by its position and the orientation; the configuration manifold lies in the special Euclidean group $\SE$. 
%
The homogeneous representation configuration manifold is given by
\begin{equation}\begin{aligned}
	\label{eq:homo}
    g = \begin{bmatrix}
    R & \pvec \\ 0 & 1
    \end{bmatrix}\!\in\!\SE.
\end{aligned}\end{equation}
%
where $R\!\in\!\SO$, $\pvec\!\in\!\mathbb{R}^3$, and $\SO\!=\!\{R\!\in\!\mathbb{R}^{3\times3}| R^TR = R R^T = I, \text{det}(R)\!=\!1\}$.

The Lie algebra of $\SO$, denoted by $\so$, defines  skew-symmetric matrices. 
%
The hat map for $\so$ is defined by $\widehat{(\cdot)}:\mathbb{R}^3\!\to\!\so$, which maps an angular velocity vector $\omega \in \mathbb{R}^3$ to its skew-symmetric cross product matrix i.e., $\hat{\omega}\!=\!-\hat{\omega}^T$ for $\omega\!\in\!\mathbb{R}^3$. Thus, for any vector $v \in \mathbb{R}^3$, $\hat{\omega} v = \omega \times v$.
%
Whereby an element in $\so$ can be mapped form a vector in $\mathbb{R}^3$ using the $\hmap\; \widehat{(\cdot)}$: $\so\!\to\!\mathbb{R}^3$.
%
The  inverse of the hat map, $\widehat{(\cdot)}$, is the $\vmap\; (\cdot)^\vee$: $\so\!\to\!\mathbb{R}^3$.
%
Similarly to $\SO$, the Lie algebra of $\SE$ is denoted by $\se$.
%
The $\hmap$ for $\se$ is defined as $\widehat{(\cdot)}$: $\mathbb{R}^6\!\to\!\se$.
%
The inverse map of hat map is defined by $\vmap\; (\cdot)^\vee$: $\se\!\to\!\mathbb{R}^6$. Thus,  
\begin{equation}\begin{aligned}
    \hat{\xi} = \begin{bmatrix}
    \hat{\omega} & v \\ 0 & 0
    \end{bmatrix}\!\in\!\se \quad \forall \xi = \begin{bmatrix} v\\ \omega \end{bmatrix}\!\in\!\mathbb{R}^6, \quad v,\omega\!\in\!\mathbb{R}^3.
\end{aligned}\end{equation}
%
%The inverse map of hat map is defined by {\it vee map}, $(\cdot)^\vee: \se \to \mathbb{R}^6$.

%For the detailed description regarding Lie group and Lie algebra, we refer to \cite{murray2017mathematical} and \cite{lynch2017modern}.

\subsection{Forward Kinematics}
We begin this subsection by noting that our interest is in robotic manipulators with revolute joints.
%
% \AR{We should introduce the matrix exponential here and we also should stick to one kind of notation $e^x$ or exp, like this}
We also use the matrix exponential given as
\begin{equation}\begin{aligned} \label{eq:matrix_exp}
    e^{A}=I + A + \tfrac{A^2}{2!} + \tfrac{A^3}{3!} + \cdots + \tfrac{A^n}{n!}, \quad A\!\in\!\mathbb{R}^{n\times n},
\end{aligned}\end{equation}
%For the manipulator kinematics, we utilize the product of exponential formulation as follows:
to describe the kinematics of the manipulator:
\begin{equation}\begin{aligned}
    g(q) = e^{\hat{\xi}_1 q_1} e^{\hat{\xi}_2 q_2} \cdots e^{\hat{\xi}_n q_n}g(0) = \begin{bmatrix}
    R(q) & \pvec(q) \\ 0 & 1
    \end{bmatrix}\!\in\!\SE
\end{aligned}\end{equation}
where $g(q)$ is the homogeneous representation~\eqref{eq:homo} of the end-effector in the spatial frame, $\xi_i\!\in\!\mathbb{R}^6$ and $q_i\!\in\!\mathbb{R}$ are a twist represented in the spatial frame and a joint angle of the $i\textsuperscript{th}$ joint, respectively, for $i\!=\!1,2,\dots, n$, and $n$ is the number of joints.
%
In addition, $g(0)$ is an initial configuration.
%
Since we are dealing with revolute joints, the joint generalized position vector is $q\!=\![q_1,\cdots,q_n]^T\!\in\!\mathbb{S}^n$.

The velocity of the end-effector in the body frame, $V^b \in \mathbb{R}^{6}$, can be calculated using following formula:
\begin{equation}\begin{aligned}
    \hat{V}^b = \begin{bmatrix}
    v^b \\ \omega^b
    \end{bmatrix} = 
    g^{-1} \dot{g}
\end{aligned}\end{equation}
i.e., $\dot{g} = g \hat{V}^b$.
%
The velocity $V^b$ can also be computed using the body Jacobian matrix $J_b(q)$ as follows:
\begin{equation}\begin{aligned}\label{eq:velo_jacobian}
    V^b = J_b(q) \dot{q}.
\end{aligned}\end{equation}
For the details about $J_b(q)$, we refer to Chap 5.1 of \cite{lynch2017modern}.

\subsection{Manipulator Dynamics}
We consider the well-known manipulator dynamics equation of motion % given by
%\begin{equation}\begin{aligned} \label{eq:robot_dynamics}
%    \underbrace{M(q)\ddot{q}}_{\in\mathbb{R}^{n\times n}} + \underbrace{C(q,\dot{q})}_{\in\mathbb{R}^{n \times n}}\dot{q} + \underbrace{G(q)}_{\in\mathbb{R}^n} = \underbrace{T}_{\in\mathbb{R}^n} + \underbrace{T_e}_{\in\mathbb{R}^n},
%\end{aligned}\end{equation}
%where $M(q)$ is the symmetric positive definite inertia matrix, $C(q,\dot{q})$ is a Coriolis matrix, $G(q)$ is a moment term from gravity, $T$ is a control input given in torque, and $T_e$ is a external torques. 
\begin{equation}\begin{aligned} \label{eq:robot_dynamics}
    M(q)\ddot{q} + C(q,\dot{q})\dot{q} + G(q) = T + T_e,
\end{aligned}\end{equation}
where $M(q)\!\in\!\mathbb{R}^{n\times n}$ is the symmetric positive definite inertia matrix, $C(q,\dot{q})\!\in\!\mathbb{R}^{n \times n}$ is a Coriolis matrix, $G(q)\!\in\!\mathbb{R}^n$ is a moment term due to gravity, $T\!\in\!\mathbb{R}^n$ is a control input given in torque, and $T_e\!\in\!\mathbb{R}^n$ is an external disturbance in torque. 
%
The $(r,s)$ element of the matrix $C(q,\dot{q})$ is %(see \cite{li1999passive}),
\begin{equation}\begin{aligned}
    C_{rs}(q,\dot{q}) = \dfrac{1}{2}\sum_{t=1}^n\left[
    \dfrac{\partial M_{rs}}{\partial q_t}\dot{q}_t +
    \dfrac{\partial M_{tr}}{\partial q_s}\dot{q}_t -
    \dfrac{\partial M_{ts}}{\partial q_r}\dot{q}_t
    \right]\!,
\end{aligned}\end{equation}
see \cite{li1999passive}.
%
The Coriolis matrix calculated in this way satisfies the property that $\dot{M}\!-\!2C$ is skew-symmetric.

==> chapters/ch3_geoCon.tex <==
\subsection{Error vector derivation}
In \cite{lee2010geometric}, the authors suggest that an error function in $\SO$ can be chosen as %follows:
\begin{equation}\begin{aligned} \label{eq:metric_original}
    \psi_R(R,R_d) = \tr(I - R_d^T R),
\end{aligned}\end{equation}
where $R\!\in\!\SO$ and $R_d\!\in\!\SO$ respectively represent the actual and desired rotation matrices.
% The error function utilized in \cite{lee2010geometric} indeed stands for the distance metric at $\SO$ as in \cite{huynh2009metrics}. 
% \AR{Note: I am not fine with the wording of the last sentence, but I have no idea how to write it better.}
%
In $\SO$, the distance metric in \eqref{eq:metric_original} can also be defined using the Frobenius norm $\|\cdot\|_F$, as proposed in \cite{huynh2009metrics},
\begin{equation}\begin{aligned}\label{eq:metric_2}
    \psi_R(R,R_d)&= \tfrac{1}{2}\|I - R_d^T R\|_F\\
    &= \tfrac{1}{2}\tr\left((I - R_d^TR)^T(I - R_d^TR)\right)\!.
\end{aligned}\end{equation}
%
%After some basic algebra, one can find out that both equations are identical, but the latter one can be extended to general matrix groups.
The formulation in \eqref{eq:metric_2} can be extended to general matrix groups.
%
Therefore,  we utilize the  Frobenius norm  to define an error function in $\SE$ as:
\begin{equation}\begin{aligned} \label{eq:err_fun}
    \Psi(\g,\gd) = \tfrac{1}{2}\|I - \gd^{-1}\g\|_F,
\end{aligned}\end{equation}
where $g \in \SE$ and $g_d \in \SE$ respectively represent
the actual and desired configurations.
%
Utilizing the homogeneous representation \eqref{eq:homo}, it follows that
\begin{equation}\begin{aligned}
    \g = \begin{bmatrix}
    R & \pvec \\
    0 & 1
    \end{bmatrix}\!, \quad \gd = \begin{bmatrix}
    R_d & \pvecd \\
    0 & 1
    \end{bmatrix}\!, \quad \g^{-1} = \begin{bmatrix}
    R^T & - R^T \pvec\\
    0 & 1
    \end{bmatrix}\!.
\end{aligned}\end{equation}
%
This leads to the equivalent formulation for the error function $\Psi(\g,\gd)$ in  \eqref{eq:err_fun}:
\begin{equation}\begin{aligned} \label{eq:err_fun_SE3}
    \Psi(\g,\gd) = \tr(I - R_d^TR) + \tfrac{1}{2}(\pvec - \pvecd)^T(\pvec - \pvecd).
\end{aligned}\end{equation}
%
This error function is related to the squared of the distance metric in $\SE$ proposed in \cite{park1995distance}, in the sense that the error function in \cite{park1995distance} is also defined as a weighed summation of metrics in $\SO$ and the Euclidean space. However, in  \cite{park1995distance} the bi-invariant metric $\| \log(R^TR_d)\|$ is utilized for $\SO$.
\JS{
In addition, the error function derived herein is the non-weighted version of the first error function of $\SE$ by \cite{bullo1999tracking}. We also emphasize that by using the Frobenius norm-induced error function, we could justify the selection of the particular error function.
}

%
% \JS{Note that this form of error function \eqref{eq:err_fun_SE3} are widely utilized as the potential energy contained in translational and rotational springs. (Maybe Controversial)}
%
It is important to note that the $\SE$ error function \eqref{eq:err_fun_SE3} is left-invariant i.e.,
\begin{equation}\label{eq:left_invariant}
    \begin{aligned}
        \Psi(g_l\g,g_l\gd) = \tfrac{1}{2}\| I - \gd^{-1}g_l^{-1}g_l\g\|_F = \Psi(g,g_d),
    \end{aligned}
\end{equation}
where $g_l\!\in\!\SE$ is an arbitrary left translation.
%
On the other hand, the right translation of the error function does not satisfy equation \eqref{eq:err_fun_SE3}.
%
Applying the right translations reads
\begin{equation}\label{eq:right_invariant}
    \begin{aligned}
        \Psi(\g g_r,\gd g_r) = \tfrac{1}{2}\| I - g_r^{-1}\gd^{-1}\g g_r\|_F \neq \Psi(g,g_d),
    \end{aligned}
\end{equation}
where $g_r\!\in\!\SE$ is an arbitrary right translation,
which confirms that the error function is left-invariant. As suggested by \cite{park1995distance}, it is natural to use body-frame coordinates for  left-invariant error metrics in $\SE$.

To calculate the error vector in $\SE$, we  perturb a configuration $\g \in \SE$ with a right translation, as was done as in \cite{lee2010geometric} for $\SO$.
\begin{equation}\begin{aligned}
    \g_{\hat{\eta}}= g e^{\hat{\eta}\epsilon}\!, \quad \eta=\begin{bmatrix}\eta_1\\ \eta_2\end{bmatrix}\!\in\!\mathbb{R}^6 \implies \hat{\eta}\!\in\!\se, \;\epsilon\!\in\!\mathbb{R},
\end{aligned}\end{equation}
where $\eta_1, \eta_2\!\in\!\mathbb{R}^3$ refer to translational and rotational components, respectively.
% is given by
%\begin{equation*}\begin{aligned}
%        \exp(\hat{\eta}\epsilon)&=I + \hat{\eta} \epsilon + \frac{(\hat{\eta} \epsilon)^2}{2!} + \frac{(\hat{\eta} \epsilon)^3}{3!} + \cdots + \frac{(\hat{\eta} \epsilon)^n}{n!}.
%\end{aligned}\end{equation*}
%where $\exp(\cdot)$ represents the matrix exponential, $\eta\!=\![\eta_1^T, \eta_2^T ]^T\!\in\!\mathbb{R}^6$, $\hat{\eta}\!\in\!\se$, and $\epsilon\!\in\!\mathbb{R}$.
%
Therefore, the configuration variation  can be represented by the homogeneous tranformation matrix
\begin{equation}\begin{aligned}
    \delta g_{\hat{\eta}} = g \hat{\eta} \implies \begin{bmatrix}
    \delta R & \delta \pvec \\
    0 & 0 
    \end{bmatrix}  = \begin{bmatrix}
    R\hat{\eta}_2 & R \eta_1 \\ 0 & 0 
    \end{bmatrix}\!\in\!T_\g\SE,
\end{aligned}\end{equation}
where $T_\g \SE$ represent tangent space of $\SE$ at configuration $\g$.
%
Expressing the error function \eqref{eq:err_fun_SE3} as
\begin{equation*}\begin{aligned}
    \Psi(g,g_d) = \dfrac{1}{2}\tr\begin{bmatrix}
    2I \!-\! R^T R_d \!-\! R_d^T R & \ast\\
    \ast & (\pvec \!-\! \pvecd)^T(\pvec \!-\! \pvecd)
    \end{bmatrix}\!,
\end{aligned}\end{equation*}
where we utilize ~$\ast$ to denote the content of irrelevant matrix elements,
%\AR{$\ast$ should be introduced here.}
%where $\ast$ symbol denotes uninterested parts of the matrix because of the trace operator. 
its perturbation can be obtained by
\begin{equation}\begin{aligned}
    \delta \Psi(\g,\gd)&=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\delta R^T R_d\!-\!R_d^T \delta R & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T \delta \pvec
    \end{bmatrix}\\
    &=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\hat{\eta}_2^T R^TR_d\!-\!R_d^T R \hat{\eta}_2 & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T R \eta_1 
    \end{bmatrix}\\
    &= -\tr(R_d^T R \hat{\eta}_2) + (\pvec\!-\!\pvecd)^T R \eta_1\\
    &= (R_d^T R - R^T R_d)^\vee \cdot \eta_2 + (\pvec - \pvecd)^T R \eta_1.
\end{aligned}\end{equation}
%where $\ast$ symbol denotes uninterested parts of the matrix because of the trace operator. 
%
We now define the \emph{position} error vector $\eg$ 
% \AR{is the naming positional correct?} 
as
\begin{equation}\begin{aligned}\label{eq:eg}
    \eg = \begin{bmatrix}
    e_p \\ e_R
    \end{bmatrix} = \begin{bmatrix}
    R^T(\pvec - \pvecd) \\
    (R_d^T R - R^T R_d)^\vee 
    \end{bmatrix},
\end{aligned}\end{equation}
so that $\delta \Psi(\g,\gd)\!=\!\eg ^T \eta$ and
\begin{equation}\begin{aligned}
    \hat{e}_g = \begin{bmatrix}
    R_d^T R - R^T R_d & R^T (\pvec - \pvecd) \\
    0 & 0 
    \end{bmatrix}.
\end{aligned}\end{equation}
%The comments on the left translational perturbation results are provided in the Appendix.~\ref{Sec:A}.
The perturbation using the left translation is included in the Appendix.~\ref{Sec:A}. However, this perturbation is not employed since the desired notation of $\eg$ is not suitable for the subsequent formulations.

As suggested in \cite{lee2010geometric}, the tangent vectors $\dot{\g}\!\in\!T_\g\SE$ and $\dot{\g}_d\!\in\!T_{\gd}\SE$ cannot be directly compared since they are not in the same tangent spaces. 
%
The desired velocity vector $V_d^b$ defined in $\gd$ can be translated into the vector $V_d^*$ in $\g$ using the following formula (See Ch 4.2 of \cite{murray2017mathematical} for the details of these steps): 
\begin{equation}\begin{aligned}
    \hat{V}_d^* = \g_{ed} \hat{V}_d^b \g_{ed}^{-1}, \text{ where } \g_{ed}\!=\!\g^{-1}\gd.
\end{aligned}\end{equation}
%
Additionally, it can be further represented as
\begin{equation}\begin{aligned}\label{eq:Ad_velo}
    V_d^* = \text{Ad}_{\g_{ed}}V_d^b, \text{ with } \text{Ad}_{\g_{ed}} = \begin{bmatrix}
   R_{ed} & \hat{\pvec}_{ed} R_{ed} \\ 0 & R_{ed}
    \end{bmatrix},
\end{aligned}\end{equation}
where $\text{Ad}_{\g_{ed}}: \mathbb{R}^6 \to \mathbb{R}^6$ is an Adjoint map. %, which is 
%\begin{equation}\begin{aligned}
%    \text{Ad}_{g} = \begin{bmatrix}
%    R & \hat{\pvec} R \\ 0 & R
%    \end{bmatrix}\!, \quad \text{with} \; g = \begin{bmatrix}
%    R & \pvec \\ 0 & 1
%    \end{bmatrix}\!.
%\end{aligned}\end{equation}
%
Based on this, we define the \emph{velocity} error vector $\ev$ as 
\begin{equation}\begin{aligned} \label{eq:ev}
    \ev\!=\!\underbrace{\begin{bmatrix}
    v^b \\ w^b \end{bmatrix}}_{V^b} \!-\! \underbrace{\begin{bmatrix}
     R^TR_d v_d\!+\!R^T R_d \hat{\omega}_d R_d^T (\pvec\!-\!\pvecd)\\
     R^T R_d \omega_d \end{bmatrix}}_{V_d^*} \!=\! \begin{bmatrix}
    e_v \\ e_\Omega \end{bmatrix}\!.
\end{aligned}\end{equation}
%
It is also worth noting that
\begin{align}
    \dot{\g} \!-\! \dot{\g}_d(\gd^{-1}\g)&\!=\! \g \hat{V}^b \!-\! \gd \hat{V}_d \gd^{-1} \g \!=\! g(\hat{V}^b \!-\! \g^{-1}\gd \hat{V}_d \gd^{-1}\g) \nonumber\\
    &= \g \hat{e}_V \in T_\g \SE,
\end{align}
which means that our velocity error vector $e_V$ can be utilized to represent the error on the tangent space at $\g$.

\subsection{Impedance control as a dissipative control}
We consider the impedance control problem as a dissipative control design. 
%
Suppose that we have a Lyapunov function in the form of the total mechanical energy given by
% \AR{Maybe change V to L for Lyapunov / makes difference between velocity V and Lyapunov function clearer} \JS{I would like to stick to it.}
\begin{equation}\begin{aligned} \label{eq:lyapunov_function}
    V(t, q,\dot{q}) = K(t, q,\dot{q}) + P(t,q), 
\end{aligned}\end{equation}
where $K$ and $P$ are respectively  the kinetic and potential energy components  of the Lyapunov function.
%
A desired property of the Lyapunov function is that it be dissipative, i.e., $\dot{V}(q,\dot{q})\!\leq\!0$. 
%
% To do so, we first define the kinetic energy part and the potential energy part of the Lyapunov function.
%
The kinetic energy component of the Lyapunov function is defined as
\begin{equation}\begin{aligned}
    K(t, q,\dot{q}) = \tfrac{1}{2}\ev^T \tilde{M}(q) \ev,
\end{aligned}\end{equation}
where $\tilde{M}(q)$ will be defined in the later in this section.
% and $J_b(q)$ is the Jacobian matrix which connects velocity in end-effector frame and the velocity of the joint angle, i.e., $V^b\!=\!J_b(q)\dot{q}$.

One easy option for the potential component of the Lyapunov function is to use a scalar multiplicative of the error function. 
%
However, recent applications such as variable impedance control require multiple and varying compliance gains in different directions \JS{\cite{zhang2021learning, martin2019variable}}. 
%
Therefore, we define a weighted version of the error function \eqref{eq:err_fun_SE3} as our potential function %$P(g,g_d)$ as follows.
\begin{equation}\begin{aligned}
    P(t,q) &= \tfrac{1}{2}\tr\left(\psi_k(\g,\g_d)^T\psi_k(\g,\g_d)\right)\!,\text{ where}\\
    \psi_k(\g,\g_d) &= \begin{bmatrix}
    \sqrt{K_o}(I -R_d^TR) & - R_d^T \sqrt{K_t}(\pvec - \pvecd)\\
    0 & 0 
    \end{bmatrix}\!,
\end{aligned}\end{equation}
$K_o\!=\!\text{diag}([k_{o1},k_{o2},k_{o3}])\!\in\!\mathbb{R}^{3\times3}$, and $K_t\!\in\!\mathbb{R}^{3\times3}$ are symmetric positive definite stiffness matrices for orientation and translation, respectively.
%
Then, using the fact that $\tr(A)\!=\!\tr(A^T)$, leads to
\begin{equation}\begin{aligned} 
    P(t,q) = \tr\!\left(K_o(I\!-\!R_d^TR)\right) + \tfrac{1}{2}(\pvec\!-\! \pvecd)^T K_t (\pvec\!-\!\pvecd).
\end{aligned}\end{equation}

The dissipative property of the impedance controller can be obtained by
\begin{equation}\begin{aligned} \label{eq:dissipative_property}
    \dfrac{dV}{dt} = -\ev^T K_d \ev,
\end{aligned}\end{equation}
with the symmetric positive definite damping matrix  $K_d\!\in\!\mathbb{R}^{6\times6}$.
%where $K_d\!\in\!\mathbb{R}^{3\times3}$ is symmetric positive definite and represents a damping matrix.
%
In order to obtain the control law, the time derivative of the Lyapunov function is considered as follows
\begin{equation}\begin{aligned} \label{eq:time_derivative_Lyapunov}
    \frac{dV}{dt} = \frac{dK}{dt} + \frac{dP}{dt}.
\end{aligned}\end{equation}
%
The first term of the right hand side of \eqref{eq:time_derivative_Lyapunov} is calculated by using \eqref{eq:Ad_velo}-\eqref{eq:ev} as
\begin{equation}\begin{aligned} \label{eq:time_derivative_kinetic}
    \frac{dK}{dt} &= \ev^T \tilde{M}(q) \dot{e}_V + \frac{1}{2}\ev^T \dot{\tilde{M}}(q) \ev\\
    &\text{with }\dot{e}_V= \dot{V}^b - \underbrace{\left(\tfrac{d}{dt}\text{Ad}_{\g_{ed}}\right)V_d^b - \text{Ad}_{\g_{ed}}\dot{V}^b_d}_{\dot{V}^*_d},
\end{aligned}\end{equation}
%
\begin{equation*}\begin{aligned}
    \frac{d}{dt}\text{Ad}_{\g_{ed}} &= \begin{bmatrix}
    \dot{R}_{ed} & \hat{\dot{p}}_{ed}R_{ed} + \hat{p}_{ed}\dot{R}_{ed} \\
    0 & \dot{R}_{ed}
    \end{bmatrix}\!,\\
    \dot{R}_{ed} &= -\hat{\omega}R^TR_d + R^T R_d \hat{\omega}_d,\\
    \dot{p}_{ed}& = -\hat{\omega}R^T(\pvec - \pvecd) + V^b - R^TR_d V_d^b.
\end{aligned}\end{equation*}
%
We define the time derivative of the desired velocity
$\dot{V}_d^*\!\triangleq\!\left(\tfrac{d}{dt}\text{Ad}_{\g_{ed}}\right)V_d^b\!-\!\text{Ad}_{\g_{ed}}\dot{V}^b_d$, so that $\dot{e}_V\!=\!\dot{V}^b\!-\!\dot{V}_d^*$.
%

\JS{
Before introducing the robot dynamics in the workspace, we note that our control design is based on the following assumption.
\begin{assum}\label{assum:1}\ \vspace{-5pt}
    \begin{enumerate}
        \item The end-effector of the manipulator and the desired trajectory lies in the reachable set $\mathcal{R}$, i.e., $p(\theta)\!\in\!\mathcal{R}\!=\!\{ p(\theta) \;|\; \forall\theta\!\in\!\mathbb{S}^n\}\!\subset\!\mathbb{R}^3$. 
        \item The end-effector lies in a region $D \subset \SE$ such that $J_b$ is full rank, i.e., non-singular. The desired trajectory is also continuously differentiable.
    \end{enumerate}
\end{assum}}
In the field of impedance control combined with operational space formulation, it is well known from \cite{khatib1987unified} that the robot dynamics \eqref{eq:robot_dynamics} can be rewritten as 
\begin{align} \label{eq:robot_dynamics_eef}
    \hspace{-5pt}\tilde{M}(q)\dot{V}^b &+ \tilde{C}(q,\dot{q})V^b + \tilde{G}(q) = \tilde{T} + \tilde{T}_e, \text{ where}\\
    \tilde{M}(q)&= J_b(q)^{-T} M(q) J_b(q)^{-1}, \nonumber\\
    \tilde{C}(q,\dot{q})&=J_b(q)^{-T}(C(q,\dot{q}) \!-\! M(q) J_b(q)^{-1}\dot{J})J_b(q)^{-1}, \nonumber\\
    \tilde{G}(q)&= J_b(q)^{-T} G(q),\; \tilde{T}= J_b(q)^{-T} T,\; \tilde{T}_e= J_b(q)^{-T} T_e.\nonumber
\end{align}
%
For compactness we use notation $\left(A^{-1}\right)^{T}\!=\!A^{-T}$.
%
Furthermore, we denote $\tilde{M}(q)$ as $\tilde{M}$, $\tilde{C}(q,\dot{q})$ as $\tilde{C}$ and $\tilde{G}(q)$ as $\tilde{G}$.
%
Then, by letting $\tilde{T}_e\!=\!0$ for control law derivation, equation~\eqref{eq:time_derivative_kinetic} can be summarized as %follows:
\begin{equation}\begin{aligned} \label{eq:delta_K}
    \frac{dK}{dt} = \ev^T &\left(\tilde{T} - \tilde{C}V^b - \tilde{G} - \tilde{M}\dot{V}_d^* - \tfrac{1}{2}\dot{\tilde{M}}\ev \right).
\end{aligned}\end{equation}
%
For the potential energy counterpart, it can be shown that 
\begin{equation}\begin{aligned} \label{eq:time_derivative_potential}
    \frac{dP}{dt} \!=\! \begin{bmatrix}
    \!e_v\! \\ \!e_\Omega\!  \end{bmatrix}^T\!
    \begin{bmatrix}
    \!K_t\! & 0 \\ 0 & \!\bar{K}_o\! \end{bmatrix} \!
    \begin{bmatrix}
    \!e_p\! \\ \!e_R\! \end{bmatrix}\!=\!\ev^T \begin{bmatrix}
    \!K_t\! & 0 \\
    0 & \!\bar{K}_o\!
    \end{bmatrix}\!\eg \!\triangleq\! \ev^T K_g \eg,
\end{aligned}\end{equation}
where $\bar{K}_o\!=\! \text{diag}\left(\left[\frac{k_{o2}+k_{o3}}{2},\frac{k_{o1}+k_{o3}}{2},\frac{k_{o1}+k_{o3}}{2}\right]\right)$.
%
The derivation of \eqref{eq:time_derivative_potential} is shown %can be found
in Appendix~\ref{Sec:A}.

The following Lemma turns out to be useful when deriving the control law.
\begin{lem} \label{lem:1}
    $\dot{\tilde{M}}\!-\!2\tilde{C}$ is skew-symmetric.
\end{lem}
\begin{pf}
    See Chap. 3.5 of \cite{lewis2003robot}.
\end{pf}
To equate \eqref{eq:time_derivative_Lyapunov} with \eqref{eq:dissipative_property}, the control law is derived as %follows.
\vspace{5pt}
\begin{equation}\begin{aligned}\label{eq:control_law}
    \tilde{T} = \tilde{M} \dot{V}_d^* + \tilde{C} V_d^* + \tilde{G} - K_g \eg - K_d \ev.
\end{aligned}\end{equation}

The following theorem shows that the proposed control law \eqref{eq:control_law} satisfies the dissipative property of the impedance controller \eqref{eq:dissipative_property}.
%
\begin{thm}
    Consider a robotic manipulator with dynamic equation of motions given by \eqref{eq:robot_dynamics}, and energy-based Lyapunov function \JS{candidate} \eqref{eq:lyapunov_function}. 
    %
    Then, the Lyapunov function of the closed-loop system with the control law \eqref{eq:control_law} satisfies dissipative property \eqref{eq:dissipative_property}, when \JS{$T_e = 0$}.
\end{thm} \vspace{-8pt}
%
\begin{pf} 
    Plugging in the control law \eqref{eq:control_law} into \eqref{eq:delta_K} and plugging in the resulting term into the Lyapunov \eqref{eq:time_derivative_Lyapunov}, and using the velocity error \eqref{eq:ev} as well as {\it Lemma \ref{lem:1}} leads to
    \begin{equation}\begin{aligned} \label{eq:deri_Lyapu}
        \frac{dV}{dt}&= \ev^T \left(\tilde{M} \dot{V}_d^* \!+\! \tilde{C}V_d^* \!-\! K_d \ev -\tilde{C}V^b \!-\! \tilde{M} \dot{V}_d^*
        \!-\! \tfrac{1}{2}\dot{\tilde{M}}\ev \right) \\
        &= \ev^T \left(\tfrac{1}{2}\dot{\tilde{M}} - \tilde{C} - K_d \right) \ev = - \ev^T K_d \ev \leq 0
    \end{aligned}\end{equation}
Which shows that the closed-loop system is at least stable in the sense of Lyapunov (SISL), and shows proper impedance behavior as proposed in \cite{kronander2016stability}.
\end{pf} \vspace{-5pt}
%
%Many  articles employ Lasalle's invariance principle on this result.
%However, rigorously speaking, the Lasalle's principle cannot be applied to the time-varying case.
\JS{One might be tempted to}
% Many articles 
employ LaSalle's invariance principle on this result, but it cannot be trivially applied to the time-varying case -- See Chap. 5.4 of \cite{sastry2013nonlinear}.
%
Therefore, \JS{following the standard strict Lyapunov analysis}, we present the asymptotic stability as presented in the following Theorem~\ref{thm:2}. 
%
% \begin{assum}\label{assum:2}\ \vspace{-5pt}
%     \begin{enumerate}
%         \item The end-effector of the manipulator and the desired trajectory lies in the reachable set $\mathcal{R}$, i.e., $p(\theta)\!\in\!\mathcal{R}\!=\!\{ p(\theta) \;|\; \forall\theta\!\in\!\mathbb{S}^n\}\!\subset\!\mathbb{R}^3$. The desired trajectory is also continuously differentiable.
%         \item In the trajectory of interest, the Jacobian matrix $J_b(q)$ is non-singular.
%     \end{enumerate}
% \end{assum}
%
\begin{thm} \label{thm:2}
    Suppose the assumption~\ref{assum:1} holds true.
    %
    Consider a robotic manipulator with dynamic equations of motion given by \eqref{eq:robot_dynamics}, and energy-based Lyapunov function \eqref{eq:lyapunov_function}.
    %
    Then, when there is no external disturbance, the closed-loop system is asymptotically stable in the reachable set $\mathcal{R}$.
\end{thm}
%
\begin{pf}
    First, to obtain the error dynamics, the position error vector $\eg$ is evaluated as
    \begin{equation}\begin{aligned}\hspace{-5pt}
        \underbrace{\frac{d}{dt}\begin{bmatrix}
        e_p \\ e_R
        \end{bmatrix}}_{\dot{e}_g} \!=\! \begin{bmatrix}
        I & \hat{e}_p \\
        0 & \tr(R^T\!R_d) I \!-\! R^T\!R_d \end{bmatrix} 
        \underbrace{\begin{bmatrix}
        e_v \\ e_\Omega \end{bmatrix}}_{\ev} \!\triangleq\! \underbrace{B(g,g_d)}_{B} e_V\!.
    \end{aligned}\end{equation}
    %
    %Then, 
    By applying the control law \eqref{eq:control_law} into \eqref{eq:robot_dynamics_eef} with $\tilde{T}_e\!=\!0$, the error dynamics is  %obtained as follows :
    \begin{equation}\begin{aligned} \label{eq:error_dynamics}
        \dot{e}_g &= B\ev \\
        \tilde{M} \dot{e}_V &= -\tilde{C}e_V - K_g \eg - K_d \ev.
    \end{aligned}\end{equation}
%    \begin{equation}\begin{aligned} \label{eq:error_dynamics}
%        \dot{e}_g &= B(g,g_d)ev \\
%        \tilde{M}(q) \dot{e}_V &= -\tilde{C}(q,\dot{q})e_V - K_g \eg - K_d \ev.
%    \end{aligned}\end{equation}
    %
    %We denotes $B(g,g_d)\!=\!B$, $\tilde{M}(q)\!=\!\tilde{M}$, and $\tilde{C}(q,\dot{q})\!=\!\tilde{C}$ for the compact notation.
    %
    Inspired by \cite{bullo1995proportional} and as suggested in \cite{lee2010geometric}, a Lyapunov function for  stability analysis can defined as follows:
    \begin{equation}\begin{aligned}
        V_2 = V + \varepsilon \eg^T \ev, \quad \varepsilon > 0.
    \end{aligned}\end{equation}
    %
    The time-derivative of $V_2$ using the Lyapunov function \eqref{eq:deri_Lyapu} the error dynamics \eqref{eq:error_dynamics} is 
    \begin{equation}\begin{aligned}
        \frac{dV_2}{dt} &= - \ev^T K_d \ev + \varepsilon \dot{e}_g^T \ev + \varepsilon \eg^T \dot{e}_V\\
        &= -\ev^T (K_d \!-\! \varepsilon B) \ev - \varepsilon \eg^T \tilde{M}^{-1}K_g \eg\\
        &\hspace{12pt}- \varepsilon \eg^T\tilde{M}^{-1}\left(\tilde{C} + K_d\right) \ev 
    \end{aligned}\end{equation}
    %
    The matrix $B$ is bounded by some constant $a$, i.e., $\|B\|\!\leq\!a$. 
    %
    This is because the reachable set is bounded, resulting in boundedness of $e_p$, and the term $(\tr(R^TR_d) I\!-\! R^TR_d)$ is found to be bounded in \cite{lee2010geometric}.
    Therefore,
    \begin{align}
        \frac{dV_2}{dt} &\leq - \evn^2(\lambda_{\min}(K_d) - \varepsilon a) -\varepsilon \tfrac{\lambda_{\min}(K_g)}{\lambda_{\max}(\tilde{M})}\egn^2 \nonumber\\
        &\hspace{12pt}- \varepsilon \left(\tfrac{\|\tilde{C}\| + \lambda_{\min}(K_d)}{\lambda_{\max}(\tilde{M})} \right)\egn\;\evn  \\
        &= -\begin{bmatrix}\egn & \evn\end{bmatrix} \begin{bmatrix}
        \varepsilon c & \varepsilon b \\
        \varepsilon b & k_d\!-\!\varepsilon a
        \end{bmatrix} \begin{bmatrix}
        \egn \\ \evn
        \end{bmatrix} \triangleq -z^T Q_\varepsilon z \nonumber
    \end{align}
    where $z\!=\!\left[\egn, \evn\right]^T\!\in\!\mathbb{R}^2$, $\lambda_{\min}(\cdot)$ and $\lambda_{\max}(\cdot)$ denotes the minimum and maximum eigenvalues, respectively, $k_d = \lambda_{\min}(K_d)$, and
    \begin{equation*}\begin{aligned}
        b \!=\! \tfrac{\|\tilde{C}\| + \lambda_{\min}(K_d)}{2\lambda_{\max}(\tilde{M})},\; c \!=\! \tfrac{\lambda_{\min}(K_g)}{\lambda_{\max}(\tilde{M})},\; Q_\varepsilon \!=\! \begin{bmatrix}
        \varepsilon c & \varepsilon b \\
        \varepsilon b & k_d \!-\!\varepsilon a
        \end{bmatrix}\!\in\!\mathbb{R}^{2\times 2}\,.
    \end{aligned}\end{equation*}
    With sufficiently large gains $K_d, K_g$ and/or taking sufficiently small $\varepsilon$, one can make $Q_\varepsilon$ positive definite. In particular, taking
    \begin{equation}\begin{aligned}
        \varepsilon < \min \left\{ \tfrac{k_d}{|a-c|}, \tfrac{k_d c}{b^2 + ac} \right\}
    \end{aligned}\end{equation}
    renders $Q_\varepsilon$ positive definite, which completes the proof.
\end{pf}
\JS{
\begin{rem}
    The control design derived herein turns out to be the modified version of the controller proposed in \cite{bullo1999tracking}. We clarify the difference as follows:
    \begin{enumerate}
        \item In \cite{bullo1999tracking}, the error function has been interpreted as the potential function, which leads to the direct derivation of the control law. On the other hand,
        we use the interpretation of distance metric, which leads to the derivation of the error vector representing the displacement between two configurations. 
        \item By utilizing the error vector in $T_g\SE$, we could find the direct connection between the Cartesian space impedance control. [{\color{red} a little bit weird] We emphasize that the error vector can be informative and insightful from an application perspective. Particularly, many techniques developed from impedance control literature, including variable impedance control \cite{martin2019variable}, can be directly applied here by changing the error representations and using body-frame Jacobian $J_b$.}
    \end{enumerate}
\end{rem}}

% {\color{red}May not be true:} We can also argue the asymptotic stability by using Lasalle's principle.
% Here, we present the following Theorem to show that the proposed controller satisfies \eqref{eq:dissipative_property}.

% \begin{theorem}
%     Consider a control law given by 
%     \begin{align}
%         \tilde{T} &= \tilde{M}(q)P(g,g_d,V_d) + \tilde{C}(q,\dot{q})V_d^* - K_g \eg - K_d \ev \nonumber \\
%         T &= J_b(q)^T \tilde{T}
%     \end{align}
%     Then, 
% \end{theorem}

==> chapters/ch3_geoCon_old.tex <==
\subsection{Error vector derivation}
In \cite{lee2010geometric}, the authors suggest that an error function in $\SO$ can be chosen as %follows:
\begin{equation}\begin{aligned} \label{eq:metric_original}
    \psi_R(R,R_d) = \tr(I - R_d^T R),
\end{aligned}\end{equation}
where $R\!\in\!\SO$ and $R_d\!\in\!\SO$ respectively represent the actual and desired rotation matrices.
% The error function utilized in \cite{lee2010geometric} indeed stands for the distance metric at $\SO$ as in \cite{huynh2009metrics}. 
% \AR{Note: I am not fine with the wording of the last sentence, but I have no idea how to write it better.}
%
In $\SO$, the distance metric in \eqref{eq:metric_original} can also be defined using the Frobenius norm $\|\cdot\|_F$, as proposed in \cite{huynh2009metrics},
\begin{equation}\begin{aligned}\label{eq:metric_2}
    \psi_R(R,R_d)&= \tfrac{1}{2}\|I - R_d^T R\|_F\\
    &= \tfrac{1}{2}\tr\left((I - R_d^TR)^T(I - R_d^TR)\right)\!.
\end{aligned}\end{equation}
%
%After some basic algebra, one can find out that both equations are identical, but the latter one can be extended to general matrix groups.
The formulation in \eqref{eq:metric_2} can be extended to general matrix groups.
%
Therefore,  we utilize the  Frobenius norm  to define an error function in $\SE$ as:
\begin{equation}\begin{aligned} \label{eq:err_fun}
    \Psi(\g,\gd) = \tfrac{1}{2}\|I - \gd^{-1}\g\|_F,
\end{aligned}\end{equation}
where $g \in \SE$ and $g_d \in \SE$ respectively represent
the actual and desired configurations.
%
Utilizing the homogeneous representation \eqref{eq:homo}, it follows that
\begin{equation}\begin{aligned}
    \g = \begin{bmatrix}
    R & \pvec \\
    0 & 1
    \end{bmatrix}\!, \quad \gd = \begin{bmatrix}
    R_d & \pvecd \\
    0 & 1
    \end{bmatrix}\!, \quad \g^{-1} = \begin{bmatrix}
    R^T & - R^T \pvec\\
    0 & 1
    \end{bmatrix}\!.
\end{aligned}\end{equation}
%
This leads to the equivalent formulation for the error function $\Psi(\g,\gd)$ in  \eqref{eq:err_fun}:
\begin{equation}\begin{aligned} \label{eq:err_fun_SE3}
    \Psi(\g,\gd) = \tr(I - R_d^TR) + \tfrac{1}{2}(\pvec - \pvecd)^T(\pvec - \pvecd).
\end{aligned}\end{equation}
%
This error function is related to the squared of the distance metric in $\SE$ proposed in \cite{park1995distance}, in the sense that the error function in \cite{park1995distance} is also defined as a weighed summation of metrics in $\SO$ and the Euclidean space. However, in  \cite{park1995distance} the bi-invariant metric $\| \log(R^TR_d)\|$ is utilized for $\SO$.

%
% \JS{Note that this form of error function \eqref{eq:err_fun_SE3} are widely utilized as the potential energy contained in translational and rotational springs. (Maybe Controversial)}
%
It is important to note that the $SE$ error function \eqref{eq:err_fun_SE3} is left-invariant i.e.,
\begin{equation}\label{eq:left_invariant}
    \begin{aligned}
        \Psi(g_l\g,g_l\gd) = \tfrac{1}{2}\| I - \gd^{-1}g_l^{-1}g_l\g\|_F = \Psi(g,g_d),
    \end{aligned}
\end{equation}
where $g_l\!\in\!\SE$ is an arbitrary left translation.
%
On the other hand, the right translation of the error function does not satisfy equation \eqref{eq:err_fun_SE3}.
%
Applying the right translations reads
\begin{equation}\label{eq:right_invariant}
    \begin{aligned}
        \Psi(\g g_r,\gd g_r) = \tfrac{1}{2}\| I - g_r^{-1}\gd^{-1}\g g_r\|_F \neq \Psi(g,g_d),
    \end{aligned}
\end{equation}
where $g_r\!\in\!\SE$ is an arbitrary right translation,
which confirms that the error function is left-invariant. As suggested by \cite{park1995distance}, it is natural to use body-frame coordinates for  left-invariant error metrics in $\SE$.

To calculate the error vector in $\SE$, we  perturb a configuration $\g \in \SE$ with a right translation, as was done as in \cite{lee2010geometric} for $\SO$.
\begin{equation}\begin{aligned}
    \g_{\hat{\eta}}= g e^{\hat{\eta}\epsilon}\!, \quad \eta=\begin{bmatrix}\eta_1\\ \eta_2\end{bmatrix}\!\in\!\mathbb{R}^6 \implies \hat{\eta}\!\in\!\se, \;\epsilon\!\in\!\mathbb{R},
\end{aligned}\end{equation}
where $\eta_1, \eta_2\!\in\!\mathbb{R}^3$ refer to translational and rotational components, respectively.
% is given by
%\begin{equation*}\begin{aligned}
%        \exp(\hat{\eta}\epsilon)&=I + \hat{\eta} \epsilon + \frac{(\hat{\eta} \epsilon)^2}{2!} + \frac{(\hat{\eta} \epsilon)^3}{3!} + \cdots + \frac{(\hat{\eta} \epsilon)^n}{n!}.
%\end{aligned}\end{equation*}
%where $\exp(\cdot)$ represents the matrix exponential, $\eta\!=\![\eta_1^T, \eta_2^T ]^T\!\in\!\mathbb{R}^6$, $\hat{\eta}\!\in\!\se$, and $\epsilon\!\in\!\mathbb{R}$.
%
Therefore, the configuration variation  can be represented by the homogeneous tranformation matrix
\begin{equation}\begin{aligned}
    \delta g_{\hat{\eta}} = g \hat{\eta} \implies \begin{bmatrix}
    \delta R & \delta \pvec \\
    0 & 0 
    \end{bmatrix}  = \begin{bmatrix}
    R\hat{\eta}_2 & R \eta_1 \\ 0 & 0 
    \end{bmatrix}\!\in\!T_\g\SE,
\end{aligned}\end{equation}
where $T_\g \SE$ represent tangent space of $\SE$ at configuration $\g$.
%
Expressing the error function \eqref{eq:err_fun_SE3} as
\begin{equation*}\begin{aligned}
    \Psi(g,g_d) = \dfrac{1}{2}\tr\begin{bmatrix}
    2I \!-\! R^T R_d \!-\! R_d^T R & \ast\\
    \ast & (\pvec \!-\! \pvecd)^T(\pvec \!-\! \pvecd)
    \end{bmatrix}\!,
\end{aligned}\end{equation*}
where we utilize ~$\ast$ to denote the content of irrelevant matrix elements,
%\AR{$\ast$ should be introduced here.}
%where $\ast$ symbol denotes uninterested parts of the matrix because of the trace operator. 
its perturbation can be obtained by
\begin{equation}\begin{aligned}
    \delta \Psi(\g,\gd)&=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\delta R^T R_d\!-\!R_d^T \delta R & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T \delta \pvec
    \end{bmatrix}\\
    &=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\hat{\eta}_2^T R^TR_d\!-\!R_d^T R \hat{\eta}_2 & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T R \eta_1 
    \end{bmatrix}\\
    &= -\tr(R_d^T R \hat{\eta}_2) + (\pvec\!-\!\pvecd)^T R \eta_1\\
    &= (R_d^T R - R^T R_d)^\vee \cdot \eta_2 + (\pvec - \pvecd)^T R \eta_1.
\end{aligned}\end{equation}
%where $\ast$ symbol denotes uninterested parts of the matrix because of the trace operator. 
%
We now define the \emph{position} error vector $\eg$ 
% \AR{is the naming positional correct?} 
as
\begin{equation}\begin{aligned}\label{eq:eg}
    \eg = \begin{bmatrix}
    e_p \\ e_R
    \end{bmatrix} = \begin{bmatrix}
    R^T(\pvec - \pvecd) \\
    (R_d^T R - R^T R_d)^\vee 
    \end{bmatrix},
\end{aligned}\end{equation}
so that $\Psi(\g,\gd)\!=\!\eg ^T \eta$ and
\begin{equation}\begin{aligned}
    \hat{e}_g = \begin{bmatrix}
    R_d^T R - R^T R_d & R^T (\pvec - \pvecd) \\
    0 & 0 
    \end{bmatrix}.
\end{aligned}\end{equation}
%The comments on the left translational perturbation results are provided in the Appendix.~\ref{Sec:A}.
The perturbation using the left translation is included in the Appendix.~\ref{Sec:A}. However, this perturbation is not employed since the desired notation of $\eg$ is not suitable for the subsequent formulations.

As suggested in \cite{lee2010geometric}, the tangent vectors $\dot{\g}\!\in\!T_\g\SE$ and $\dot{\g}_d\!\in\!T_{\gd}\SE$ cannot be directly compared since they are not in the same tangent spaces. 
%
The desired velocity vector $V_d^b$ defined in $\gd$ can be translated into the vector $V_d^*$ in $\g$ using the following formula (See Ch 4.2 of \cite{murray2017mathematical} for the details of these steps): 
\begin{equation}\begin{aligned}
    \hat{V}_d^* = \g_{ed} \hat{V}_d^b \g_{ed}^{-1}, \text{ where } \g_{ed}\!=\!\g^{-1}\gd.
\end{aligned}\end{equation}
%
Additionally, it can be further represented as
\begin{equation}\begin{aligned}\label{eq:Ad_velo}
    V_d^* = \text{Ad}_{\g_{ed}}V_d^b, \text{ with } \text{Ad}_{\g_{ed}} = \begin{bmatrix}
   R_{ed} & \hat{\pvec}_{ed} R_{ed} \\ 0 & R_{ed}
    \end{bmatrix},
\end{aligned}\end{equation}
where $\text{Ad}_{\g_{ed}}: \mathbb{R}^6 \to \mathbb{R}^6$ is an Adjoint map. %, which is 
%\begin{equation}\begin{aligned}
%    \text{Ad}_{g} = \begin{bmatrix}
%    R & \hat{\pvec} R \\ 0 & R
%    \end{bmatrix}\!, \quad \text{with} \; g = \begin{bmatrix}
%    R & \pvec \\ 0 & 1
%    \end{bmatrix}\!.
%\end{aligned}\end{equation}
%
Based on this, we define the \emph{velocity} error vector $\ev$ as 
\begin{equation}\begin{aligned} \label{eq:ev}
    \ev\!=\!\underbrace{\begin{bmatrix}
    v^b \\ w^b \end{bmatrix}}_{V^b} \!-\! \underbrace{\begin{bmatrix}
     R^TR_d v_d\!+\!R^T R_d \hat{\omega}_d R_d^T (\pvec\!-\!\pvecd)\\
     R^T R_d \omega_d \end{bmatrix}}_{V_d^*} \!=\! \begin{bmatrix}
    e_v \\ e_\Omega \end{bmatrix}\!.
\end{aligned}\end{equation}
%
It is also worth noting that
\begin{align}
    \dot{\g} \!-\! \dot{\g}_d(\gd^{-1}\g)&\!=\! \g \hat{V}^b \!-\! \gd \hat{V}_d \gd^{-1} \g \!=\! g(\hat{V}^b \!-\! \g^{-1}\gd \hat{V}_d \gd^{-1}\g) \nonumber\\
    &= \g \hat{e}_V \in T_\g \SE,
\end{align}
which means that our velocity error vector $e_V$ can be utilized to represent the error on the tangent space at $\g$.

\subsection{Impedance control as a dissipative control}
We consider the impedance control problem as a dissipative control design. 
%
Suppose that we have a Lyapunov function in the form of the total mechanical energy given by
% \AR{Maybe change V to L for Lyapunov / makes difference between velocity V and Lyapunov function clearer} \JS{I would like to stick to it.}
\begin{equation}\begin{aligned} \label{eq:lyapunov_function}
    V(t, q,\dot{q}) = K(t, q,\dot{q}) + P(t,q), 
\end{aligned}\end{equation}
where $K$ and $P$ are respectively  the kinetic and potential energy components  of the Lyapunov function.
%
A desired property of the Lyapunov function is that it be dissipative, i.e., $\dot{V}(q,\dot{q})\!\leq\!0$. 
%
% To do so, we first define the kinetic energy part and the potential energy part of the Lyapunov function.
%
The kinetic energy component of the Lyapunov function is defined as
\begin{equation}\begin{aligned}
    K(t, q,\dot{q}) = \tfrac{1}{2}\ev^T \tilde{M}(q) \ev,
\end{aligned}\end{equation}
where $\tilde{M}(q)$ will be defined in the later in this section.
% and $J_b(q)$ is the Jacobian matrix which connects velocity in end-effector frame and the velocity of the joint angle, i.e., $V^b\!=\!J_b(q)\dot{q}$.

One easy option for the potential component of the Lyapunov function is to use a scalar multiplicative of the error function. 
%
However, recent applications of impedance control require multiple and varying compliance gains in different directions. 
%
Therefore, we define a weighted version of the error function \eqref{eq:err_fun_SE3} as our potential function %$P(g,g_d)$ as follows.
\begin{equation}\begin{aligned}
    P(t,q) &= \tfrac{1}{2}\tr\left(\psi_k(\g,\g_d)^T\psi_k(\g,\g_d)\right)\!,\text{ where}\\
    \psi_k(\g,\g_d) &= \begin{bmatrix}
    \sqrt{K_o}(I -R_d^TR) & - R_d^T \sqrt{K_t}(\pvec - \pvecd)\\
    0 & 0 
    \end{bmatrix}\!,
\end{aligned}\end{equation}
$K_o\!=\!\text{diag}([k_{o1},k_{o2},k_{o3}])\!\in\!\mathbb{R}^3$, and $K_t\!\in\!\mathbb{R}^3$ are symmetric positive definite stiffness matrices for orientation and translation, respectively.
%
Then, using the fact that $\tr(A)\!=\!\tr(A^T)$, leads to
\begin{equation}\begin{aligned} 
    P(t,q) = \tr\!\left(K_o(I\!-\!R_d^TR)\right) + \tfrac{1}{2}(\pvec\!-\! \pvecd)^T K_t (\pvec\!-\!\pvecd).
\end{aligned}\end{equation}

The dissipative property of the impedance controller can be obtained by
\begin{equation}\begin{aligned} \label{eq:dissipative_property}
    \dfrac{dV}{dt} = -\ev^T K_d \ev,
\end{aligned}\end{equation}
with the symmetric positive definite damping matrix  $K_d\!\in\!\mathbb{R}^{6\times6}$.
%where $K_d\!\in\!\mathbb{R}^{3\times3}$ is symmetric positive definite and represents a damping matrix.
%
In order to obtain the control law, the time derivative of the Lyapunov function is considered as follows
\begin{equation}\begin{aligned} \label{eq:time_derivative_Lyapunov}
    \frac{dV}{dt} = \frac{dK}{dt} + \frac{dP}{dt}.
\end{aligned}\end{equation}
%
The first term of the right hand side of \eqref{eq:time_derivative_Lyapunov} is calculated by using \eqref{eq:Ad_velo}-\eqref{eq:ev} as
\begin{equation}\begin{aligned} \label{eq:time_derivative_kinetic}
    \frac{dK}{dt} &= \ev^T \tilde{M}(q) \dot{e}_V + \frac{1}{2}\ev^T \dot{\tilde{M}}(q) \ev\\
    &\text{with }\dot{e}_V= \dot{V}^b - \underbrace{\left(\tfrac{d}{dt}\text{Ad}_{\g_{ed}}\right)V_d^b - \text{Ad}_{\g_{ed}}\dot{V}^b_d}_{\dot{V}^*_d},
\end{aligned}\end{equation}
%
\begin{equation*}\begin{aligned}
    \frac{d}{dt}\text{Ad}_{\g_{ed}} &= \begin{bmatrix}
    \dot{R}_{ed} & \hat{\dot{p}}_{ed}R_{ed} + \hat{p}_{ed}\dot{R}_{ed} \\
    0 & \dot{R}_{ed}
    \end{bmatrix}\!,\\
    \dot{R}_{ed} &= -\hat{\omega}R^TR_d + R^T R_d \hat{\omega}_d,\\
    \dot{p}_{ed}& = -\hat{\omega}R^T(\pvec - \pvecd) + V^b - R^TR_d V_d^b.
\end{aligned}\end{equation*}
%
We define the time derivative of the desired velocity
$\dot{V}_d^*\!\triangleq\!\left(\tfrac{d}{dt}\text{Ad}_{\g_{ed}}\right)V_d^b\!-\!\text{Ad}_{\g_{ed}}\dot{V}^b_d$, so that $\dot{e}_V\!=\!\dot{V}^b\!-\!\dot{V}_d^*$.
%

In the field of impedance control, it is well known from \cite{khatib1987unified} that the robot dynamics \eqref{eq:robot_dynamics} can be rewritten as 
\begin{align} \label{eq:robot_dynamics_eef}
    \hspace{-5pt}\tilde{M}(q)\dot{V}^b &+ \tilde{C}(q,\dot{q})V^b + \tilde{G}(q) = \tilde{T} + \tilde{T}_e, \text{ where}\\
    \tilde{M}(q)&= J_b(q)^{-T} M(q) J_b(q)^{-1}, \nonumber\\
    \tilde{C}(q,\dot{q})&=J_b(q)^{-T}(C(q,\dot{q}) \!-\! M(q) J_b(q)^{-1}\dot{J})J_b(q)^{-1}, \nonumber\\
    \tilde{G}(q)&= J_b(q)^{-T} G(q),\; \tilde{T}= J_b(q)^{-T} T,\; \tilde{T}_e= J_b(q)^{-T} T_e.\nonumber
\end{align}
%
For compactness we use notation $\left(A^{-1}\right)^{T}\!=\!A^{-T}$.
%
Furthermore, we denote $\tilde{M}(q)$ as $\tilde{M}$, $\tilde{C}(q,\dot{q})$ as $\tilde{C}$ and $\tilde{G}(q)$ as $\tilde{G}$.
%
Then, by letting $\tilde{T}_e\!=\!0$ for control law derivation, equation~\eqref{eq:time_derivative_kinetic} can be summarized as %follows:
\begin{equation}\begin{aligned} \label{eq:delta_K}
    \frac{dK}{dt} = \ev^T &\left(\tilde{T} - \tilde{C}V^b - \tilde{G} - \tilde{M}\dot{V}_d^* - \tfrac{1}{2}\dot{\tilde{M}}\ev \right).
\end{aligned}\end{equation}
%
For the potential energy counterpart, it can be shown that 
\begin{equation}\begin{aligned} \label{eq:time_derivative_potential}
    \frac{dP}{dt} \!=\! \begin{bmatrix}
    \!e_v\! \\ \!e_\Omega\!  \end{bmatrix}^T\!
    \begin{bmatrix}
    \!K_t\! & 0 \\ 0 & \!\bar{K}_o\! \end{bmatrix} \!
    \begin{bmatrix}
    \!e_p\! \\ \!e_R\! \end{bmatrix}\!=\!\ev^T \begin{bmatrix}
    \!K_t\! & 0 \\
    0 & \!\bar{K}_o\!
    \end{bmatrix}\!\eg \!\triangleq\! \ev^T K_g \eg,
\end{aligned}\end{equation}
where $\bar{K}_o\!=\! \text{diag}\left(\left[\frac{k_{o2}+k_{o3}}{2},\frac{k_{o1}+k_{o3}}{2},\frac{k_{o1}+k_{o3}}{2}\right]\right)$.
%
The derivation of \eqref{eq:time_derivative_potential} is shown %can be found
in Appendix~\ref{Sec:A}.

The following Lemma turns out to be useful when deriving the control law.
\begin{lem} \label{lem:1}
    $\dot{\tilde{M}}\!-\!2\tilde{C}$ is skew-symmetric.
\end{lem}
\begin{pf}
    See Chap. 3.5 of \cite{lewis2003robot}.
\end{pf}
To equate \eqref{eq:time_derivative_Lyapunov} with \eqref{eq:dissipative_property}, the control law is derived as %follows.
\vspace{5pt}
\begin{equation}\begin{aligned}\label{eq:control_law}
    \tilde{T} = \tilde{M} \dot{V}_d^* + \tilde{C} V_d^* + \tilde{G} - K_g \eg - K_d \ev.
\end{aligned}\end{equation}

The following theorem shows that the proposed control law \eqref{eq:control_law} satisfies the dissipative property of the impedance controller \eqref{eq:dissipative_property}.
%
\begin{thm}
    Consider a robotic manipulator with dynamic equation of motions given by \eqref{eq:robot_dynamics}, and energy-based Lyapunov function \eqref{eq:lyapunov_function}. 
    %
    Then, the Lyapunov function of the closed-loop system with the control law \eqref{eq:control_law} satisfies dissipative property \eqref{eq:dissipative_property}, when there is no external disturbance.
\end{thm}
%
\begin{pf}
    Plugging in the control law \eqref{eq:control_law} into \eqref{eq:delta_K} and plugging in the resulting term into the Lyapunov \eqref{eq:time_derivative_Lyapunov}, and using the velocity error \eqref{eq:ev} as well as {\it Lemma \ref{lem:1}} leads to
    \begin{equation}\begin{aligned} \label{eq:deri_Lyapu}
        \frac{dV}{dt}&= \ev^T \left(\tilde{M} \dot{V}_d^* \!+\! \tilde{C}V_d^* \!-\! K_d \ev -\tilde{C}V^b \!-\! \tilde{M} \dot{V}_d^*
        \!-\! \tfrac{1}{2}\dot{\tilde{M}}\ev \right) \\
        &= \ev^T \left(\tfrac{1}{2}\dot{\tilde{M}} - \tilde{C} - K_d \right) \ev = - \ev^T K_d \ev
    \end{aligned}\end{equation}
\end{pf}
Which shows that the closed-loop system is at least stable in the sense of Lyapunov (SISL), and shows proper impedance behavior as proposed in \cite{kronander2016stability}.
%
%Many  articles employ Lasalle's invariance principle on this result.
%However, rigorously speaking, the Lasalle's principle cannot be applied to the time-varying case. 
Many articles employ LaSalle's invariance principle on this result, but it cannot be trivially applied to the time-varying case -- See Chap. 5.4 of \cite{sastry2013nonlinear}.
%
Therefore, we present the asymptotic stability as presented in the following Theorem~\ref{thm:2}. 
%
Note that our main results is based on
\begin{assum}\label{assum:1}\ \vspace{-5pt}
    \begin{enumerate}
        \item The end-effector of the manipulator and the desired trajectory lies in the reachable set $\mathcal{R}$, i.e., $p(\theta)\!\in\!\mathcal{R}\!=\!\{ p(\theta) \;|\; \forall\theta\!\in\!\mathbb{S}^n\}\!\subset\!\mathbb{R}^3$. The desired trajectory is also continuously differentiable.
        \item In the trajectory of interest, the Jacobian matrix $J_b(q)$ is non-singular.
    \end{enumerate}
\end{assum}
%
\begin{thm} \label{thm:2}
    Suppose the assumption~\ref{assum:1} holds true.
    %
    Consider a robotic manipulator with dynamic equations of motion given by \eqref{eq:robot_dynamics}, and energy-based Lyapunov function \eqref{eq:lyapunov_function}.
    %
    Then, when there is no external disturbance, the closed-loop system is asymptotically stable in the reachable set $\mathcal{R}$.
\end{thm}
%
\begin{pf}
    First, to obtain the error dynamics, the position error vector $\eg$ is evaluated as
    \begin{equation}\begin{aligned}\hspace{-5pt}
        \underbrace{\frac{d}{dt}\begin{bmatrix}
        e_p \\ e_R
        \end{bmatrix}}_{\dot{e}_g} \!=\! \begin{bmatrix}
        I & \hat{e}_p \\
        0 & \tr(R^T\!R_d) I \!-\! R^T\!R_d \end{bmatrix} 
        \underbrace{\begin{bmatrix}
        e_v \\ e_\Omega \end{bmatrix}}_{\ev} \!\triangleq\! \underbrace{B(g,g_d)}_{B} e_V\!.
    \end{aligned}\end{equation}
    %
    %Then, 
    By applying the control law \eqref{eq:control_law} into \eqref{eq:robot_dynamics_eef} with $\tilde{T}_e\!=\!0$, the error dynamics is  %obtained as follows :
    \begin{equation}\begin{aligned} \label{eq:error_dynamics}
        \dot{e}_g &= B\ev \\
        \tilde{M} \dot{e}_V &= -\tilde{C}e_V - K_g \eg - K_d \ev.
    \end{aligned}\end{equation}
%    \begin{equation}\begin{aligned} \label{eq:error_dynamics}
%        \dot{e}_g &= B(g,g_d)ev \\
%        \tilde{M}(q) \dot{e}_V &= -\tilde{C}(q,\dot{q})e_V - K_g \eg - K_d \ev.
%    \end{aligned}\end{equation}
    %
    %We denotes $B(g,g_d)\!=\!B$, $\tilde{M}(q)\!=\!\tilde{M}$, and $\tilde{C}(q,\dot{q})\!=\!\tilde{C}$ for the compact notation.
    %
    Inspired by \cite{bullo1995proportional} and as suggested in \cite{lee2010geometric}, a Lyapunov function for  stability analysis can defined as follows:
    \begin{equation}\begin{aligned}
        V_2 = V + \varepsilon \eg^T \ev, \quad \varepsilon > 0.
    \end{aligned}\end{equation}
    %
    The time-derivative of $V_2$ using the Lyapunov function \eqref{eq:deri_Lyapu} the error dynamics \eqref{eq:error_dynamics} is 
    \begin{equation}\begin{aligned}
        \frac{dV_2}{dt} &= - \ev^T K_d \ev + \varepsilon \dot{e}_g^T \ev + \varepsilon \eg^T \dot{e}_V\\
        &= -\ev^T (K_d \!-\! \varepsilon B) \ev - \varepsilon \eg^T \tilde{M}^{-1}K_g \eg\\
        &\hspace{12pt}- \varepsilon \eg^T\tilde{M}^{-1}\left(\tilde{C} + K_d\right) \ev 
    \end{aligned}\end{equation}
    %
    The matrix $B$ is bounded by some constant $a$, i.e., $\|B\|\!\leq\!a$. 
    %
    This is because the reachable set is bounded, resulting in boundedness of $e_p$, and the term $(\tr(R^TR_d) I\!-\! R^TR_d)$ is found to be bounded in \cite{lee2010geometric}.
    Therefore,
    \begin{align}
        \frac{dV_2}{dt} &\leq - \evn^2(\lambda_{\min}(K_d) - \varepsilon a) -\varepsilon \tfrac{\lambda_{\min}(K_g)}{\lambda_{\max}(\tilde{M})}\egn^2 \nonumber\\
        &\hspace{12pt}- \varepsilon \left(\tfrac{\|\tilde{C}\| + \lambda_{\min}(K_d)}{\lambda_{\max}(\tilde{M})} \right)\egn\;\evn  \\
        &= -\begin{bmatrix}\egn & \evn\end{bmatrix} \begin{bmatrix}
        \varepsilon c & \varepsilon b \\
        \varepsilon b & k_d\!-\!\varepsilon a
        \end{bmatrix} \begin{bmatrix}
        \egn \\ \evn
        \end{bmatrix} \triangleq -z^T Q_\varepsilon z \nonumber
    \end{align}
    where $z\!=\!\left[\egn, \evn\right]^T\!\in\!\mathbb{R}^2$, $\lambda_{\min}(\cdot)$ and $\lambda_{\max}(\cdot)$ denotes the minimum and maximum eigenvalues, respectively, $k_d = \lambda_{\min}(K_d)$, and
    \begin{equation*}\begin{aligned}
        b \!=\! \tfrac{\|\tilde{C}\| + \lambda_{\min}(K_d)}{2\lambda_{\max}(\tilde{M})},\; c \!=\! \tfrac{\lambda_{\min}(K_g)}{\lambda_{\max}(\tilde{M})},\; Q_\varepsilon \!=\! \begin{bmatrix}
        \varepsilon c & \varepsilon b \\
        \varepsilon b & k_d \!-\!\varepsilon a
        \end{bmatrix}\!\in\!\mathbb{R}^{2\times 2}\,.
    \end{aligned}\end{equation*}
    With sufficiently large gains $K_d, K_g$ and/or taking sufficiently small $\varepsilon$, one can make $Q_\varepsilon$ positive definite. In particular, taking
    \begin{equation}\begin{aligned}
        \varepsilon < \min \left\{ \tfrac{k_d}{|a-c|}, \tfrac{k_d c}{b^2 + ac} \right\}
    \end{aligned}\end{equation}
    renders $Q_\varepsilon$ positive definite, which completes the proof.
\end{pf}


% {\color{red}May not be true:} We can also argue the asymptotic stability by using Lasalle's principle.
% Here, we present the following Theorem to show that the proposed controller satisfies \eqref{eq:dissipative_property}.

% \begin{theorem}
%     Consider a control law given by 
%     \begin{align}
%         \tilde{T} &= \tilde{M}(q)P(g,g_d,V_d) + \tilde{C}(q,\dot{q})V_d^* - K_g \eg - K_d \ev \nonumber \\
%         T &= J_b(q)^T \tilde{T}
%     \end{align}
%     Then, 
% \end{theorem}

==> chapters/ch3_geoCon_renew.tex <==
\subsection{Error vector derivation}
In \cite{lee2010geometric}, the authors suggest that an error function in $\SO$ can be chosen as %follows:
\begin{equation}\begin{aligned} \label{eq:metric_original}
    \psi_R(R,R_d) = \tr(I - R_d^T R),
\end{aligned}\end{equation}
where $R\!\in\!\SO$ and $R_d\!\in\!\SO$ respectively represent the actual and desired rotation matrices.
% The error function utilized in \cite{lee2010geometric} indeed stands for the distance metric at $\SO$ as in \cite{huynh2009metrics}. 
% \AR{Note: I am not fine with the wording of the last sentence, but I have no idea how to write it better.}
%
In $\SO$, the distance metric in \eqref{eq:metric_original} can also be defined using the Frobenius norm $\|\cdot\|_F$, as proposed in \cite{huynh2009metrics},
\begin{equation}\begin{aligned}\label{eq:metric_2}
    \psi_R(R,R_d)&= \tfrac{1}{2}\|I - R_d^T R\|_F\\
    &= \tfrac{1}{2}\tr\left((I - R_d^TR)^T(I - R_d^TR)\right)\!.
\end{aligned}\end{equation}
%
%After some basic algebra, one can find out that both equations are identical, but the latter one can be extended to general matrix groups.
The formulation in \eqref{eq:metric_2} can be extended to general matrix groups.
%
Therefore,  we utilize the  Frobenius norm  to define an error function in $\SE$ as:
\begin{equation}\begin{aligned} \label{eq:err_fun}
    \Psi(\g,\gd) = \tfrac{1}{2}\|I - \gd^{-1}\g\|_F,
\end{aligned}\end{equation}
where $g \in \SE$ and $g_d \in \SE$ respectively represent
the actual and desired configurations.
%
Utilizing the homogeneous representation \eqref{eq:homo}, it follows that
\begin{equation}\begin{aligned}
    \g = \begin{bmatrix}
    R & \pvec \\
    0 & 1
    \end{bmatrix}\!, \quad \gd = \begin{bmatrix}
    R_d & \pvecd \\
    0 & 1
    \end{bmatrix}\!, \quad \g^{-1} = \begin{bmatrix}
    R^T & - R^T \pvec\\
    0 & 1
    \end{bmatrix}\!.
\end{aligned}\end{equation}
%
This leads to the equivalent formulation for the error function $\Psi(\g,\gd)$ in  \eqref{eq:err_fun}:
\begin{equation}\begin{aligned} \label{eq:err_fun_SE3}
    \Psi(\g,\gd) = \tr(I - R_d^TR) + \tfrac{1}{2}(\pvec - \pvecd)^T(\pvec - \pvecd).
\end{aligned}\end{equation}
%
This error function is related to the squared of the distance metric in $\SE$ proposed in \cite{park1995distance}, in the sense that the error function in \cite{park1995distance} is also defined as a weighed summation of metrics in $\SO$ and the Euclidean space. However, in  \cite{park1995distance} the bi-invariant metric $\| \log(R^TR_d)\|$ is utilized for $\SO$.
In addition, the error function derived herein is the non-weighted version of one of the error functions proposed by \cite{bullo1999tracking}. We also emphasize that, by using the Frobenius norm-induced error function, we could justify the selection of the weighted error function in \cite{bullo1999tracking}.
It is important to note that the $\SE$ error function \eqref{eq:err_fun_SE3} is left-invariant i.e.,
\begin{equation}\label{eq:left_invariant}
    \begin{aligned}
        \Psi(g_l\g,g_l\gd) = \tfrac{1}{2}\| I - \gd^{-1}g_l^{-1}g_l\g\|_F = \Psi(g,g_d),
    \end{aligned}
\end{equation}
where $g_l\!\in\!\SE$ is an arbitrary left translation.
%
On the other hand, the right translation of the error function does not satisfy equation \eqref{eq:err_fun_SE3}.
%
Applying the right translations reads
\begin{equation}\label{eq:right_invariant}
    \begin{aligned}
        \Psi(\g g_r,\gd g_r) = \tfrac{1}{2}\| I - g_r^{-1}\gd^{-1}\g g_r\|_F \neq \Psi(g,g_d),
    \end{aligned}
\end{equation}
where $g_r\!\in\!\SE$ is an arbitrary right translation,
which confirms that the error function is left-invariant. As suggested by \cite{park1995distance}, it is natural to use body-frame coordinates for  left-invariant error metrics in $\SE$.

To calculate the error vector in $\SE$, we  perturb a configuration $\g \in \SE$ with a right translation, as was done as in \cite{lee2010geometric} for $\SO$.
\begin{equation}\begin{aligned}
    \g_{\hat{\eta}}= g e^{\hat{\eta}\epsilon}\!, \quad \eta=\begin{bmatrix}\eta_1\\ \eta_2\end{bmatrix}\!\in\!\mathbb{R}^6 \implies \hat{\eta}\!\in\!\se, \;\epsilon\!\in\!\mathbb{R},
\end{aligned}\end{equation}
where $\eta_1, \eta_2\!\in\!\mathbb{R}^3$ refer to translational and rotational components, respectively.
% is given by
%\begin{equation*}\begin{aligned}
%        \exp(\hat{\eta}\epsilon)&=I + \hat{\eta} \epsilon + \frac{(\hat{\eta} \epsilon)^2}{2!} + \frac{(\hat{\eta} \epsilon)^3}{3!} + \cdots + \frac{(\hat{\eta} \epsilon)^n}{n!}.
%\end{aligned}\end{equation*}
%where $\exp(\cdot)$ represents the matrix exponential, $\eta\!=\![\eta_1^T, \eta_2^T ]^T\!\in\!\mathbb{R}^6$, $\hat{\eta}\!\in\!\se$, and $\epsilon\!\in\!\mathbb{R}$.
%
Therefore, the configuration variation  can be represented by the homogeneous transformation matrix
\begin{equation}\begin{aligned}
    \delta g_{\hat{\eta}} = g \hat{\eta} \implies \begin{bmatrix}
    \delta R & \delta \pvec \\
    0 & 0 
    \end{bmatrix}  = \begin{bmatrix}
    R\hat{\eta}_2 & R \eta_1 \\ 0 & 0 
    \end{bmatrix}\!\in\!T_\g\SE,
\end{aligned}\end{equation}
where $\hat{\eta}_2 \in \so$ and $T_\g \SE$ represent tangent space of $\SE$ at configuration $\g$.
%
Expressing the error function \eqref{eq:err_fun_SE3} as
\begin{equation*}\begin{aligned}
    \Psi(g,g_d) = \dfrac{1}{2}\tr\begin{bmatrix}
    2I \!-\! R^T R_d \!-\! R_d^T R & \ast\\
    \ast & (\pvec \!-\! \pvecd)^T(\pvec \!-\! \pvecd)
    \end{bmatrix}\!,
\end{aligned}\end{equation*}
where we utilize ~$\ast$ to denote the content of irrelevant matrix elements,
%\AR{$\ast$ should be introduced here.}
%where $\ast$ symbol denotes uninterested parts of the matrix because of the trace operator. 
its perturbation can be obtained by
\begin{equation}\begin{aligned} \label{eq:perturbation_of_error_metric}
    \delta \Psi(\g,\gd)&=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\delta R^T R_d\!-\!R_d^T \delta R & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T \delta \pvec
    \end{bmatrix}\\
    &=\!\dfrac{1}{2}\tr\!\begin{bmatrix}\!
    -\hat{\eta}_2^T R^TR_d\!-\!R_d^T R \hat{\eta}_2 & \ast
    % \eta_2 - R_d^T R \eta_2 - \hat{\eta}_1 R^T (\pvec - \pvecd)
    \\
    \ast &  2(\pvec\!-\!\pvecd)^T R \eta_1 
    \end{bmatrix}\\
    &= -\tr(R_d^T R \hat{\eta}_2) + (\pvec\!-\!\pvecd)^T R \eta_1\\
    &= (R_d^T R - R^T R_d)^\vee \cdot \eta_2 + (\pvec - \pvecd)^T R \eta_1.
\end{aligned}\end{equation}
%where $\ast$ symbol denotes uninterested parts of the matrix because of the trace operator. 
%
We now define the \emph{position} error vector $\eg$ 
% \AR{is the naming positional correct?} 
as
\begin{equation}\begin{aligned}\label{eq:eg}
    \eg = \begin{bmatrix}
    e_p \\ e_R
    \end{bmatrix} = \begin{bmatrix}
    R^T(\pvec - \pvecd) \\
    (R_d^T R - R^T R_d)^\vee 
    \end{bmatrix} \in \mathbb{R}^6,
\end{aligned}\end{equation}
so that $\delta \Psi(\g,\gd)\!=\!\eg ^T \eta$ and
\begin{equation}\begin{aligned}
    \hat{e}_g = \begin{bmatrix}
    R_d^T R - R^T R_d & R^T (\pvec - \pvecd) \\
    0 & 0 
    \end{bmatrix} \in \se.
\end{aligned}\end{equation}
As suggested in \cite{lee2010geometric}, the tangent vectors $\dot{\g}\!\in\!T_\g\SE$ and $\dot{\g}_d\!\in\!T_{\gd}\SE$ cannot be directly compared since they are not in the same tangent spaces. 
%
The desired velocity vector $V_d^b$ defined in $\gd$ can be translated into the vector $V_d^*$ in $\g$ using the following formula (See Ch 4.2 of \cite{murray2017mathematical} for the details of these steps): 
\begin{equation}\begin{aligned}
    \hat{V}_d^* = \g_{ed} \hat{V}_d^b \g_{ed}^{-1}, \text{ where } \g_{ed}\!=\!\g^{-1}\gd.
\end{aligned}\end{equation}
%
Additionally, it can be further represented as
\begin{equation}\begin{aligned}\label{eq:Ad_velo}
    V_d^* = \text{Ad}_{\g_{ed}}V_d^b, \text{ with } \text{Ad}_{\g_{ed}} = \begin{bmatrix}
   R_{ed} & \hat{\pvec}_{ed} R_{ed} \\ 0 & R_{ed}
    \end{bmatrix},
\end{aligned}\end{equation}
where $\text{Ad}_{\g_{ed}}: \mathbb{R}^6 \to \mathbb{R}^6$ is an Adjoint map, $R_{ed}\! =\! R^T R_d$, and $p_{ed} \!=\!-R^T(p\! -\! p_d)$. %, which is 
%\begin{equation}\begin{aligned}
%    \text{Ad}_{g} = \begin{bmatrix}
%    R & \hat{\pvec} R \\ 0 & R
%    \end{bmatrix}\!, \quad \text{with} \; g = \begin{bmatrix}
%    R & \pvec \\ 0 & 1
%    \end{bmatrix}\!.
%\end{aligned}\end{equation}
%
Based on this, we define the \emph{velocity} error vector $\ev$ as 
\begin{equation}\begin{aligned} \label{eq:ev}
    \ev\!=\!\underbrace{\begin{bmatrix}
    v^b \\ w^b \end{bmatrix}}_{V^b} \!-\! \underbrace{\begin{bmatrix}
     R^TR_d v_d\!+\!R^T R_d \hat{\omega}_d R_d^T (\pvec\!-\!\pvecd)\\
     R^T R_d \omega_d \end{bmatrix}}_{V_d^*} \!=\! \begin{bmatrix}
    e_v \\ e_\Omega \end{bmatrix}\!.
\end{aligned}\end{equation}
%
It is also worth noting that
\begin{align}
    \dot{\g} \!-\! \dot{\g}_d(\gd^{-1}\g)&\!=\! \g \hat{V}^b \!-\! \gd \hat{V}_d \gd^{-1} \g \!=\! g(\hat{V}^b \!-\! \g^{-1}\gd \hat{V}_d \gd^{-1}\g) \nonumber\\
    &= \g \hat{e}_V \in T_\g \SE,
\end{align}
which means that the velocity error vector $e_V$ can be utilized to represent the error on the tangent space at $\g$.

\subsection{Impedance control as a dissipative control}
We consider the impedance control problem as a dissipative control design. 
%
\JS{Suppose that we have a Lyapunov function in a form that is similar to the total mechanical energy of the system
% \AR{Maybe change V to L for Lyapunov / makes difference between velocity V and Lyapunov function clearer} \JS{I would like to stick to it.}
\begin{equation}\begin{aligned} \label{eq:lyapunov_function}
    V(t, q, \dot{q}) = K(t, q, \dot{q}) + P(t,q), 
\end{aligned}\end{equation}
where $K$ and $P$ are the kinetic and potential energy components  of the Lyapunov function. Note that using total mechanical energy as a Lyapunov function is quite standard, as first proposed by \cite{koditschek1989application}}.
%
A desired property of the Lyapunov function is a dissipativity, i.e., $\dot{V}(t, q, \dot{q})\!\leq\!0$. 
%
% To do so, we first define the kinetic energy part and the potential energy part of the Lyapunov function.
%
The kinetic energy component of the Lyapunov function can be  defined as follows
\begin{equation}\begin{aligned}
    K(t, q, q_d, \dot{q}, \dot{q}_d) = \tfrac{1}{2}\ev^T \tilde{M}(q) \ev,
\end{aligned}\end{equation}
where $\tilde{M}(q)$ is defined in \eqref{eq:robot_dynamics_eef} and $\ev$ is defined in \eqref{eq:ev}.
% and $J_b(q)$ is the Jacobian matrix which connects velocity in end-effector frame and the velocity of the joint angle, i.e., $V^b\!=\!J_b(q)\dot{q}$.

One easy option for the potential component of the Lyapunov function is to use a scalar multiplicative of the error function $\Psi(\g,\gd)$ in \eqref{eq:err_fun_SE3}. 
%
However, recent applications such as variable impedance control require multiple and varying compliance gains in different directions \JS{\cite{zhang2021learning, martin2019variable}}. 
%
Therefore, we define a weighted version of the error function \eqref{eq:err_fun_SE3} as our potential function %$P(g,g_d)$ as follows.
\begin{equation}\begin{aligned}\label{eq:potential_function}
    P(t,q, q_d) &= \tfrac{1}{2}\tr\left(\psi_k(\g,\g_d)^T\psi_k(\g,\g_d)\right)\!,\text{ where}\\
    \psi_k(\g,\g_d) &= \begin{bmatrix}
    \sqrt{K_R}(I -R_d^TR) & - \sqrt{K_p} R_d^T (\pvec - \pvecd)\\
    0 & 0 
    \end{bmatrix}\!,
\end{aligned}\end{equation}
\JS{$K_R\! \in \!\mathbb{R}^{3\times3}$, and $K_p\!\in\!\mathbb{R}^{3\times3}$ are symmetric positive definite stiffness matrices for orientation and translation, respectively.}
%
Then, using the fact that $\tr(A)\!=\!\tr(A^T)$, leads to
\JS{
\begin{equation}\begin{aligned} 
    P(t,q, q_d)\! =\! \tr\!\left(K_R(I\!-\!R_d^TR)\right)\! +\! \tfrac{1}{2}(\pvec\!-\! \pvecd)^T R_d K_p R_d^T (\pvec\!-\!\pvecd).
\end{aligned}\end{equation}}
\JS{The potential function \eqref{eq:potential_function} is the second version of the multiple $\SE$ error function alternatives presented in Table.~1 of \cite{bullo1999tracking}.
Using the error vector $e_g$ and $e_V$, an intuitive impedance control law that resembles conventional impedance controllers, can be formulated as follows:
\begin{equation}\begin{aligned} \label{eq:intuitive_impedance}
    \tilde{T} = \tilde{M} \dot{V}_d^* + \tilde{C} V_d^* + \tilde{G} - K_g \eg - K_d \ev
\end{aligned}\end{equation}
where $K_g = \text{blkdiag}(K_p, K_R)$. Here, the $K_g \eg$ term can be interpreted as the spring force in $T_g^*\SE$, i.e., $f_g = K_g e_g$. 
However, the control action from \eqref{eq:intuitive_impedance} is not in the gradient direction of \eqref{eq:lyapunov_function}. 
Therefore, as shown in \cite{bullo1999tracking}, the elastic force $f_g$ induced from the potential function \eqref{eq:potential_function}, such that $f_g\!\in\! T_g^*\SE$, should be utilized and is given as follows:
\begin{equation}\begin{aligned} \label{eq:geometric_impedance}
    f_g = \begin{bmatrix}
    f_p \\ f_R
    \end{bmatrix} =\begin{bmatrix}
    R^T R_d K_p R_d^T (\pvec - \pvecd)\\
    (K_R R_d^T R - R^T R_d K_R)^\vee
    \end{bmatrix}
\end{aligned}\end{equation} 
The derivation of \eqref{eq:geometric_impedance} is presented in the Appendix~\ref{Sec:A}.
Using \eqref{eq:geometric_impedance}, a geometric impedance control law on $\SE$ is given by
\JS{
\begin{equation}\begin{aligned}\label{eq:control_law}
    \tilde{T} = \tilde{M} \dot{V}_d^* + \tilde{C} V_d^* + \tilde{G} - f_g - K_d \ev.
\end{aligned}\end{equation}}
\vspace{-12pt}
\begin{rem} Comparison between the control laws  \eqref{eq:intuitive_impedance} and \eqref{eq:control_law}. \\
    The translational part of the elastic force in \eqref{eq:control_law} can be evaluated as follows.
    \begin{equation}\begin{aligned}
        f_p &= R^T R_d K_p R_d^T(p - p_d)\\
        &= R^T R_d K_p R_d^T R R_T(p - p_d) = \tilde{K}_p e_p
    \end{aligned}\end{equation}
    where $\tilde{K}_p = R^T R_d K_p R_d^T R$. Further letting $R_{ed} = R^T R_d$, it can be denoted by $\tilde{K}_p = R_{ed} K_p R_{ed}^T$ and represents the coordinate transformation of the stiffness matrix. In \eqref{eq:intuitive_impedance}, the stiffness is represented in the end-effector frame, while it is represented in the desired frame in the \eqref{eq:control_law}. Therefore, the translational part in \eqref{eq:intuitive_impedance} and \eqref{eq:control_law} can be considered as equivalent.
    However, the rotational components of the control laws  \eqref{eq:intuitive_impedance} and \eqref{eq:control_law} are equivalent  when $K_R = k_R I$ and $k_R \in \mathbb{R}_+$ is a scalar.
    %or $K_R = k_R\hat{w}$ with $\left.R^TR_d w = R^T R_d\right.$, i.e. $w \in \mathbb{R}^3$ is the efective axis of rotation of $R^TR_d$.
\end{rem}
}
\JS{
The proposed control design is based on the following assumption.
\begin{assum} \label{assum:2}
    The end-effector of the manipulator and the desired trajectory lies in the reachable set $\mathcal{R}$, i.e., $p(\theta)\!\in\!\mathcal{R}\!=\!\{ p(\theta) \;|\; \forall\theta\!\in\!\mathbb{S}^n\}\!\subset\!\mathbb{R}^3$. 
    The desired trajectory is also continuously differentiable.
\end{assum}
}
The dissipative property of the impedance controller can be obtained by
\begin{equation}\begin{aligned} \label{eq:dissipative_property}
    \dfrac{dV}{dt} = -\ev^T K_d \ev,
\end{aligned}\end{equation}
with the symmetric positive definite damping matrix  $K_d\!\in\!\mathbb{R}^{6\times6}$.
%where $K_d\!\in\!\mathbb{R}^{3\times3}$ is symmetric positive definite and represents a damping matrix.
%
In order to obtain the control law, the time derivative of the Lyapunov function is considered as follows
\begin{equation}\begin{aligned} \label{eq:time_derivative_Lyapunov}
    \frac{dV}{dt} = \frac{dK}{dt} + \frac{dP}{dt}.
\end{aligned}\end{equation}
%
The first term of the right hand side of \eqref{eq:time_derivative_Lyapunov} is calculated by using \eqref{eq:Ad_velo}-\eqref{eq:ev} as
\begin{equation}\begin{aligned} \label{eq:time_derivative_kinetic}
    \frac{dK}{dt} &= \ev^T \tilde{M}(q) \dot{e}_V + \frac{1}{2}\ev^T \dot{\tilde{M}}(q) \ev\\
    &\text{with }\dot{e}_V= \dot{V}^b - \underbrace{\left(\tfrac{d}{dt}\text{Ad}_{\g_{ed}}\right)V_d^b - \text{Ad}_{\g_{ed}}\dot{V}^b_d}_{\dot{V}^*_d},
\end{aligned}\end{equation}
%
\begin{equation*}\begin{aligned}
    \frac{d}{dt}\text{Ad}_{\g_{ed}} &= \begin{bmatrix}
    \dot{R}_{ed} & \hat{\dot{p}}_{ed}R_{ed} + \hat{p}_{ed}\dot{R}_{ed} \\
    0 & \dot{R}_{ed}
    \end{bmatrix}\!,\\
    \dot{R}_{ed} &= -\hat{\omega}R^TR_d + R^T R_d \hat{\omega}_d,\\
    \dot{p}_{ed}& = -\hat{\omega}R^T(\pvec - \pvecd) + V^b - R^TR_d V_d^b.
\end{aligned}\end{equation*}
%
We define the time derivative of the desired velocity
$\dot{V}_d^*\!\triangleq\!\left(\tfrac{d}{dt}\text{Ad}_{\g_{ed}}\right)V_d^b\!-\!\text{Ad}_{\g_{ed}}\dot{V}^b_d$, so that $\dot{e}_V\!=\!\dot{V}^b\!-\!\dot{V}_d^*$.
%
Then, by letting $\tilde{T}_e\!=\!0$ for control law derivation, equation~\eqref{eq:time_derivative_kinetic} can be summarized as %follows:
\begin{equation}\begin{aligned} \label{eq:delta_K}
    \frac{dK}{dt} = \ev^T &\left(\tilde{T} - \tilde{C}V^b - \tilde{G} - \tilde{M}\dot{V}_d^* - \tfrac{1}{2}\dot{\tilde{M}}\ev \right).
\end{aligned}\end{equation}
%
For the potential energy counterpart, it can be shown that 
\JS{
\begin{equation}\begin{aligned} \label{eq:time_derivative_potential}
    \frac{dP}{dt} = f_g ^T e_V.
\end{aligned}\end{equation}
}
%
The derivation of \eqref{eq:time_derivative_potential} is shown %can be found
in Appendix~\ref{Sec:A}.

The following Lemma turns out to be useful when deriving the control law.
\begin{lem} \label{lem:1}
    $\dot{\tilde{M}}\!-\!2\tilde{C}$ is skew-symmetric.
\end{lem}
\begin{pf}
    See Chap. 3.5 of \cite{lewis2003robot}.
\end{pf}
The following theorem shows that the proposed control law \eqref{eq:control_law} satisfies the dissipative property of the impedance controller \eqref{eq:dissipative_property}.
%
\begin{thm}
    Suppose assumptions~\ref{assum:1} and \ref{assum:2} hold true.
    Consider a robotic manipulator with the dynamic equation of motions given by \eqref{eq:robot_dynamics} and energy-based Lyapunov function \JS{candidate} \eqref{eq:lyapunov_function}.
    %
    Then, the Lyapunov function of the closed-loop system with the control law \eqref{eq:control_law} satisfies dissipative property \eqref{eq:dissipative_property}, when \JS{$T_e = 0$}.
\end{thm} \vspace{-8pt}
%
\begin{pf} 
    Plugging in the control law \eqref{eq:control_law} into \eqref{eq:delta_K} and plugging in the resulting term into the Lyapunov \eqref{eq:time_derivative_Lyapunov}, and using the velocity error \eqref{eq:ev} as well as {\it Lemma \ref{lem:1}} leads to
    \begin{align} \label{eq:deri_Lyapu}
        \frac{dV}{dt}&= \ev^T \left(\tilde{M} \dot{V}_d^* \!+\! \tilde{C}V_d^* \!-\! K_d \ev -\tilde{C}V^b \!-\! \tilde{M} \dot{V}_d^*
        \!-\! \tfrac{1}{2}\dot{\tilde{M}}\ev \right) \nonumber \\
        &= \ev^T \left(\tfrac{1}{2}\dot{\tilde{M}} - \tilde{C} - K_d \right) \ev = - \ev^T K_d \ev \leq 0
    \end{align}
Which shows that the closed-loop system is at least stable in the sense of Lyapunov (SISL), and shows proper impedance behavior as proposed in \cite{kronander2016stability}.
\end{pf} \vspace{-5pt}
%
%Many  articles employ Lasalle's invariance principle on this result.
%However, rigorously speaking, the Lasalle's principle cannot be applied to the time-varying case.
LaSalle's invariance principle cannot be employed on this result since it cannot be trivially applied to the time-varying case -- See Chap. 5.4 of \cite{sastry2013nonlinear}.
%
Therefore, \JS{following the standard strict Lyapunov analysis}, we present the asymptotic stability as presented in the following Theorem~\ref{thm:2}. 
%
% \begin{assum}\label{assum:2}\ \vspace{-5pt}
%     \begin{enumerate}
%         \item The end-effector of the manipulator and the desired trajectory lies in the reachable set $\mathcal{R}$, i.e., $p(\theta)\!\in\!\mathcal{R}\!=\!\{ p(\theta) \;|\; \forall\theta\!\in\!\mathbb{S}^n\}\!\subset\!\mathbb{R}^3$. The desired trajectory is also continuously differentiable.
%         \item In the trajectory of interest, the Jacobian matrix $J_b(q)$ is non-singular.
%     \end{enumerate}
% \end{assum}
%
\begin{thm} \label{thm:2}
    Suppose the assumptions~\ref{assum:1} and ~\ref{assum:2} hold true.
    %
    Consider a robotic manipulator with dynamic equations of motion given by \eqref{eq:robot_dynamics}, and energy-based Lyapunov function \eqref{eq:lyapunov_function}.
    %
    Then, when $T_e\! =\! 0$, \JS{the equilibrium point $\left.g(t)\! =\! g_d(t)\right.$, such that $f_g \!=\! 0$, of the closed-loop system} is asymptotically stable in the reachable set $\mathcal{R}$.
\end{thm}
%
\begin{pf}
    % First, to obtain the error dynamics, the position error vector $\eg$ is evaluated as
    \JS{First, the time derivative of $f_g = [f_p^T, f_R^T]^T$ term is calculated as follows.
    \begin{align}\hspace{-5pt} \label{eq:f_g_dot}
        \frac{d}{dt}\begin{bmatrix}
        f_p \\ f_R
        \end{bmatrix} \!&=\! \begin{bmatrix}
        R^TR_d K_p R_d^T R & \hat{f}_p \\
        0 & \tr(R^T R_d K_R) I\! -\! R^T R_d K_R \end{bmatrix} 
        \begin{bmatrix}
        e_v \\ e_\Omega \end{bmatrix} \nonumber\\ 
        &\triangleq\! B_K(g,g_d) e_V\!.
    \end{align}
    We denote $B_K(g,g_d) = B_K$ for the compactness of the notation. The derivation of \eqref{eq:f_g_dot} is presented in the Appendix~\ref{Sec:A}.
    }
    %
    By applying the control law \eqref{eq:control_law} into \eqref{eq:robot_dynamics_eef} with $\tilde{T}_e\!=\!0$, the error dynamics is  %obtained as follows :
    \JS{
    \begin{equation}\begin{aligned} \label{eq:error_dynamics}
        \dot{f}_g &= B_K\ev \\
        \tilde{M} \dot{e}_V &= -\tilde{C}e_V - f_g - K_d \ev.
    \end{aligned}\end{equation}}
%    \begin{equation}\begin{aligned} \label{eq:error_dynamics}
%        \dot{e}_g &= B(g,g_d)ev \\
%        \tilde{M}(q) \dot{e}_V &= -\tilde{C}(q,\dot{q})e_V - K_g \eg - K_d \ev.
%    \end{aligned}\end{equation}
    %
    %We denotes $B(g,g_d)\!=\!B$, $\tilde{M}(q)\!=\!\tilde{M}$, and $\tilde{C}(q,\dot{q})\!=\!\tilde{C}$ for the compact notation.
    %
    Inspired by \cite{bullo1995proportional} and as suggested in \cite{lee2010geometric}, a Lyapunov function \JS{candidate $W$} for  stability analysis can defined as follows:
    \JS{
    \begin{equation}\begin{aligned}
        W = V + \varepsilon f_g^T \ev, \quad \varepsilon > 0.
    \end{aligned}\end{equation}}
    %
    The time-derivative of $W$ using the Lyapunov function \eqref{eq:deri_Lyapu} the error dynamics \eqref{eq:error_dynamics} is 
    \JS{
    \begin{equation}\begin{aligned}
        \frac{dW}{dt} &= - \ev^T K_d \ev + \varepsilon \dot{f}_g^T \ev + \varepsilon f_g^T \dot{e}_V\\
        &= -\ev^T (K_d \!-\! \varepsilon B_K) \ev - \varepsilon f_g^T \tilde{M}^{-1}f_g\\
        &\hspace{12pt}- \varepsilon f_g^T\tilde{M}^{-1}\left(\tilde{C} + K_d\right) \ev 
    \end{aligned}\end{equation}
    }
    %
    The matrix \JS{$B_K$} is bounded by some constant $a$, i.e., \JS{$\left.\|B\|_K\!\leq\!a\right.$} 
    %
    \JS{This is because the reachable set is bounded, resulting in boundedness of $f_p$, and the term $(\tr(R^T R_d K_R) I\! -\! R^T R_d K_R)$ is bounded as similarly as proposed in \cite{lee2010geometric}.}
    Therefore,
    \JS{
    \begin{align}
        \frac{dW}{dt} &\leq - \evn^2(\lambda_{\min}(K_d) - \varepsilon a) -\varepsilon \tfrac{1}{\lambda_{\max}(\tilde{M})}\|f_g\|_2^2 \nonumber\\
        &\hspace{12pt}- \varepsilon \left(\tfrac{\|\tilde{C}\| + \lambda_{\min}(K_d)}{\lambda_{\max}(\tilde{M})} \right)\|f_g\|_2\;\evn  \\
        &= -\begin{bmatrix}\|f_g\|_2 & \evn\end{bmatrix} \begin{bmatrix}
        \varepsilon c & \varepsilon b \\
        \varepsilon b & k_d\!-\!\varepsilon a
        \end{bmatrix} \begin{bmatrix}
        \|f_g\|_2 \\ \evn
        \end{bmatrix} \triangleq -z^T Q_\varepsilon z \nonumber
    \end{align}}
    where \JS{$z\!=\!\left[\|f_g\|_2, \evn\right]^T\!\in\!\mathbb{R}^2$,} $\lambda_{\min}(\cdot)$ and $\lambda_{\max}(\cdot)$ denotes the minimum and maximum eigenvalue of the matrix, respectively, $k_d = \lambda_{\min}(K_d)$, and
    \begin{equation*}\begin{aligned}
        b \!=\! \tfrac{\|\tilde{C}\| + \lambda_{\min}(K_d)}{2\lambda_{\max}(\tilde{M})},\; c \!=\! \tfrac{1}{\lambda_{\max}(\tilde{M})},\; Q_\varepsilon \!=\! \begin{bmatrix}
        \varepsilon c & \varepsilon b \\
        \varepsilon b & k_d \!-\!\varepsilon a
        \end{bmatrix}\!\in\!\mathbb{R}^{2\times 2}\,.
    \end{aligned}\end{equation*}
    With sufficiently large gains $K_d, K_g$ and/or taking sufficiently small $\varepsilon$, one can make $Q_\varepsilon$ positive definite. In particular, taking
    \begin{equation}\begin{aligned}
        \varepsilon < \min \left\{ \tfrac{k_d}{|a-c|}, \tfrac{k_d c}{b^2 + ac} \right\}
    \end{aligned}\end{equation}
    renders $Q_\varepsilon$ positive definite, which completes the proof.
\end{pf}
\begin{rem}
Connection with Matrosov's theorem \\
Beginning from the result \eqref{eq:deri_Lyapu}, Matrosov's theorem can also be utilized as \cite{loria2005nested, paden1988globally}. In particular, \cite{paden1988globally} utilized $\dot{V}$ term as the auxiliary function, and \cite{loria2005nested} utilized the inner product of position and velocity errors as the auxiliary function. The main concept of both approaches is looking into the time derivative of positional error. In our stability analysis, the coupling term $f_g^T e_V$ provides a time derivative of the positional error. Therefore, a strict Lyapunov analysis with the coupling term and Matrosov's theorem can be considered equivalent.
\end{rem}
\begin{rem}
We can also show the stability of intuitive impedance control law \eqref{eq:intuitive_impedance}, but it is omitted due to the page limit.
\end{rem}
% \JS{
% \begin{rem}
%     The control design derived herein turns out to be the modified version of the controller proposed in \cite{bullo1999tracking}. We clarify the difference as follows:
%     \begin{enumerate}
%         \item In \cite{bullo1999tracking}, the error function has been interpreted as the potential function, which leads to the direct derivation of the control law. On the other hand,
%         we use the interpretation of distance metric, which leads to the derivation of the error vector representing the displacement between two configurations. 
%         \item By utilizing the error vector in $T_g\SE$, we could find the direct connection between the Cartesian space impedance control. [{\color{red} a little bit weird] We emphasize that the error vector can be informative and insightful from an application perspective. Particularly, many techniques developed from impedance control literature, including variable impedance control \cite{martin2019variable}, can be directly applied here by changing the error representations and using body-frame Jacobian $J_b$.}
%     \end{enumerate}
% \end{rem}}

==> chapters/ch4_sim.tex <==
% We utilize the UR5e model as our robot model, which are designed using Robotic Toolbox Matlab (\cite{corke2002robotics}) in the matlab environment.
% \AR{I would suggest: We utilize the UR5e model [\cite{corke2002robotics}] implemented in matlab [version; cite matlab].}
We utilize the UR5e robot model implemented in Matlab~R2021a using \cite{corke2002robotics}. %(version R2021a).
%
As a benchmark, we use conventional impedance control, which does not consider geometrical aspects, while allowing comparable comparison to our version from \cite{robosuite2020, ochoa2021impedance, shaw2022rmps}. 
\JS{In particular, the control law utilized for the benchmark is as follows:
\begin{equation} \label{eq:conventional_impedance}
    \begin{aligned}
        \tilde{T}^s = \tilde{M}^s\dot{V}_d + \tilde{C}^s V + \tilde{G}^s - K_g e_g^s - K_d {e}_V^s
    \end{aligned}
\end{equation}
where $\tilde{M}^s$, $\tilde{C}^s$, and $\tilde{G}^s$ can be obtained by replacing $J_b$ to $J_s$, a spatial Jacobian matrix, from \eqref{eq:robot_dynamics_eef}, and $\tilde{T}^s = J_s^{-T}T$. In addition, the spatial error vector $e_g^s$ is defined as 
\begin{equation}
    \begin{aligned}
         e_g^s &= [
         (e_p^s)^T, \; (e_R^s)^T
         ]^T, \quad \text{where}\\
        e_p^s &= x - x_d,\\
        e_R^s &= (r_{d_1} \times r_1 + r_{d_2} \times r_2 + r_{d_3}\times r_3),
    \end{aligned}
\end{equation}
with $R = [r_1, r_2, r_3]$ and $R_d = [r_{d_1}, r_{d_2}, r_{d_3}]$. Likewise, the spatial velocity error $e_V^s$ is
\begin{equation}
    \begin{aligned}
        e_V^s = \begin{bmatrix}
            v^s \\ \omega^s
        \end{bmatrix} - \begin{bmatrix}
            \dot{p}_d \\ \omega_d^s
        \end{bmatrix} = V^s - V_d^s,
    \end{aligned}
\end{equation}
where the spatial velocity is obtained by $V^s = J_s \dot{q}$. Note that this controller is identical to the one proposed in \cite{caccavale1999six} where the only difference is the representation of the rotational error $e_R^s$.
}

\JS{
The simulations are conducted for two cases: 1. Multi-point regulation task scenario, 2. Dynamic trajectory with rapid motion tracking scenario. 
For the fair comparison, we set the same desired impedance $K_g$ and $K_d$ to both controllers, and also let both controllers start at the same initial conditions. The desired impedance in both scenarios are set as
\begin{equation}\begin{aligned}
    K_g = \text{diag}\left([k_p,k_p,k_p,k_o,k_o,k_o]\right), \quad K_d = k_d I
    %K_d &= \text{diag}([k_d,k_d,k_d,k_d,k_d,k_d])
\end{aligned}\end{equation}
where $k_p\!=\!k_o\!=\!100$ and $k_d\!=\!50$. 

\subsection{Multi-point regulation task}
The initial condition in this scenario is
\begin{equation*}\begin{aligned}
    q(0) &= [0.1721,-1.0447,1.6729,-0.6282,0.1721,0]^T,\\
    \dot{q}(0) &= [0,0,0,0,0,0]^T,
\end{aligned}\end{equation*}
so that the initial end-effector pose would be
\begin{equation*}
    \begin{aligned}
        p_0 = [-0.5, -0.3, 0.2]^T, \quad R_0 = \begin{bmatrix}
        1 & 0 & 0\\ 0 & 0 & \!-\!1 \\ 0 & 1 & 0
        \end{bmatrix}.
    \end{aligned}
\end{equation*}
In this scenario, the desired poses are selected as
% \begin{equation*}
%     \begin{aligned}
%         p_d &= [-0.4, 0.3, 0.2]^T, \; R_d = R_{d_1}, \quad \text{for}\; 0 \leq t < 3\\
%         p_d &= [-0.4, -0.3, 0.2]^T, \; R_d = R_{d_2}, \quad \text{for}\; 3 \leq t < 6\\
%         p_d &= [-0.6, -0.3, 0.2]^T, \; R_d = R_{d_1}, \quad \text{for}\; 6 \leq t < 9\\
%         p_d &= [-0.6, 0.3, 0.2]^T, \; R_d = R_{d_2}, \quad \text{for}\; 9 \leq t < 12\\
%         p_d &= [-0.4, 0.3, 0.2]^T, \; R_d = R_{d_1}, \quad \text{for}\; 12 \leq t \leq 15
%     \end{aligned}
% \end{equation*}
\begin{equation*}
    \begin{aligned}
        \begin{array}{lll}
        p_d = [-0.4, 0.3, 0.2]^T, & R_d = R_{d_1}, & \;\;\text{for}\; 0 \leq t < 3\\
        p_d = [-0.4, -0.3, 0.2]^T, & R_d = R_{d_2}, & \;\;\text{for}\; 3 \leq t < 6\\
        p_d = [-0.6, -0.3, 0.2]^T, & R_d = R_{d_1}, & \;\;\text{for}\; 6 \leq t < 9\\
        p_d = [-0.6, 0.3, 0.2]^T, & R_d = R_{d_2}, & \;\;\text{for}\; 9 \leq t < 12\\
        p_d = [-0.4, 0.3, 0.2]^T, & R_d = R_{d_1}, & \;\;\text{for}\; 12 \leq t \leq 15 \\
        \end{array}
    \end{aligned}
\end{equation*}
with 
\begin{equation*}
    \begin{aligned}
        R_{d_1} = \begin{bmatrix}
        0 & -1 & 0\\
        0 & 0 & -1 \\
        1 & 0 & 0\\
        \end{bmatrix}, \quad R_{d_2}  = \begin{bmatrix}
        1 & 0 & 0\\
        0 & 0 & -1 \\
        0 & 1 & 0\\
        \end{bmatrix}.
    \end{aligned}
\end{equation*}
The trajectory tracking results in $x$, $y$, and $z$ coordinates are plotted in Fig.~\ref{fig:comparison_xyz_regulation}. In Fig.~\ref{fig:err_fun_regulation}, the error function \eqref{eq:err_fun_SE3} is shown for this scenario. The root-mean-squared values for the Cartesian errors and error functions are presented in Tab.~\ref{table:rms_of_errors}. As can be seen in the results, the proposed control design showed equivalent control performance in the Cartesian coordinate. On the other hand, the proposed control showed far enhanced performance in reducing initial errors, especially in the rotational part. }
\begin{figure}[b!]
    %\centering
    %\includegraphics[width=\columnwidth]{figures/comparison_xyz.eps}
    \vspace{-5pt}
    \hspace{-8pt}
    \input{figures/comparison_xyz_regulation2.tex}
    \vspace{-20pt}
    \caption{The simulation results in $x$, $y$, and $z$ coordinates for the step input scenario for the proposed and benchmark approach are plotted.}
    \label{fig:comparison_xyz_regulation}
\end{figure}
\begin{figure}
    %\centering
    %\includegraphics[width=\columnwidth]{figures/error_func.eps}
    \vspace{-5pt}
    \hspace{-6pt}
     \input{figures/error_func_regulation2.tex}
     \vspace{-20pt}
    \caption{Error function  \eqref{eq:err_fun_SE3} for the resulting trajectories for the step input scenario.}
    \label{fig:err_fun_regulation}
\end{figure}
%
\begin{table}[b!]
  \caption{Performance metrics in RMS values for multi-point regulation scenario}
  \label{table:rms_of_errors}
  \scriptsize
  \centering%
  \begin{tabu}[width=\columnwidth]{%
      c| c | c
    }
    \toprule
    Performance Metrics & Benchmark & Proposed\\
    \midrule
    $\text{RMS}(x(t) - x_d(t))$ & 0.0489 & 0.0476\\
    $\text{RMS}(y(t) - y_d(t))$ & 0.0158 & 0.0157\\
    $\text{RMS}(z(t) - z_d(t))$ & 0.0067 & 0.0049\\
    $\text{RMS}(\Psi(g(t),g_d(t))$ &0.5500 & 0.4067\\
    \bottomrule
  \end{tabu}
\end{table}

\JS{
\subsection{Trajectory tracking}
The initial point in this scenario is selected as
\begin{equation*}\begin{aligned}
    q(0) &= [0.4,-0.5,0.4,0.6,-0.5,0.2]^T,\\
    \dot{q}(0) &= [0,0,0,0,0,0]^T.
\end{aligned}\end{equation*}
The desired trajectories are
\begin{equation} \begin{aligned}
    p_d(t) = \begin{bmatrix}
    -0.52 - 0.2 \cos{\pi t}\\
    0.2 \sin{\pi t}\\
    0.2 + 0.1 \sin{0.5\pi t}
    \end{bmatrix}, \quad R_d(t) = R_0
\end{aligned} \end{equation}
In order to further evaluate performance in the dynamic trajectory tracking task, we define the following dynamic error function as follows:
\begin{equation} \label{eq:dyn_err_fun_SE3}
    \begin{aligned}
        \Phi(g,g_d,e_V) = \Psi(g,g_d) + e_V^{T}e_V 
    \end{aligned}
\end{equation}
In Fig.~\ref{fig:comparison_xyz_tracking}, the Cartesian trajectory tracking results are plotted. The error function \eqref{eq:err_fun_SE3} and \eqref{eq:dyn_err_fun_SE3} for the trajectory tracking tasks are presented in Fig.~\ref{fig:error_func_tracking} and Fig.~\ref{fig:dynamic_cost_tracking}, respectively. The RMS values for the performance metrics are shown in Tab.~\ref{table:rms_of_errors_tracking}. As can be shown in the results, the proposed control and the benchmark approach showed similar trajectory tracking performance in the Cartesian coordinate. However, similar to the previous scenario, the proposed control law showed enhanced performance in reducing the initial errors especially in orientation, as can be observed in Fig.~\ref{fig:error_func_tracking}, \ref{fig:dynamic_cost_tracking}. This is mainly because the benchmark control tries to reduce the similar potential function separately in translational and orientational direction, while the proposed control approach reduce the translational and orientational error in the combined manner.
}
\begin{figure}[t!]
    %\centering
    %\includegraphics[width=\columnwidth]{figures/comparison_xyz.eps}
    \vspace{-5pt}
    \hspace{-8pt}
    \input{figures/comparison_xyz_tracking.tex}
    \vspace{-20pt}
    \caption{The trajectory tracking results in $x$, $y$, and $z$ coordinates for the proposed and benchmark approach are plotted.}
    \label{fig:comparison_xyz_tracking}
\end{figure}
\begin{figure}[h]
    %\centering
    %\includegraphics[width=\columnwidth]{figures/comparison_xyz.eps}
    \vspace{-5pt}
    \hspace{-8pt}
    \input{figures/error_func_tracking.tex}
    \vspace{-20pt}
    \caption{Error function \eqref{eq:err_fun_SE3} for the resulting trajectories for the trajectory tracking.}
    \label{fig:error_func_tracking}
\end{figure}
\begin{figure}[h]
    %\centering
    %\includegraphics[width=\columnwidth]{figures/comparison_xyz.eps}
    \vspace{-5pt}
    \hspace{-8pt}
    \input{figures/dynamic_cost_tracking.tex}
    \vspace{-20pt}
    \caption{Dynamic error function \eqref{eq:dyn_err_fun_SE3} for the resulting trajectories for the trajectory tracking.}
    \label{fig:dynamic_cost_tracking}
\end{figure}
\begin{table}[b!]
  \caption{Performance metrics in RMS values for the dynamic trajectory tracking scenario}
  \label{table:rms_of_errors_tracking}
  \scriptsize
  \centering%
  \begin{tabu}[width=\columnwidth]{%
      c| c | c
    }
    \toprule
    Performance Metrics & Benchmark & Proposed\\
    \midrule
    $\text{RMS}(x(t) - x_d(t))$ & 0.0521 & 0.0439\\
    $\text{RMS}(y(t) - y_d(t))$ & 0.0131 & 0.0134\\
    $\text{RMS}(z(t) - z_d(t))$ & 0.0218 & 0.0234\\
    $\text{RMS}(\Psi(g(t),g_d(t))$ &0.2007 & 0.1615\\
    $\text{RMS}(\Phi(g(t),g_d(t),e_V(t))$ &17.95 & 13.71\\
    \bottomrule
  \end{tabu}
\end{table}

The Matlab code for the implementation of the controller proposed in this paper is provided in: \url{https://github.com/Joohwan-Seo/Geometric-Impedance-Control-Public}.\\
%
Few remarks on the actual implementation are provided.
\begin{rem} 
    From the implementation perspective, the normal PD control given by
    $\tilde{T}\!=\!-K_g \eg \!-\! K_d \ev$
    can be utilized when the Jacobin matrix is numerically near singular.
    %
    This implies that even without dynamic parameters and solving inverse kinematics, we can solve the end-effector positioning problem, which has already been emphasized in an earlier work 
    \cite{hogan1985impedance}.
    %
    % This means that we may not need to solve for the inverse kinematics without any dynamic parameters, which has been already emphasized in an earlier of the work \cite{hogan1985impedance}.
% In the implementation perspective, the normal PD control given by 
%         \begin{align} \label{eq:PD_control}
%             \tilde{T} = -K_g \eg - K_d \ev 
%         \end{align}
%         can be utilized when the Jacobin matrix is numerically near singular. 
\end{rem}

% \begin{figure}
%     %\centering
%     \vspace{-5pt}
%     \hspace{-8pt}
%     \input{figures/trajectory_3d.tex}
%     \vspace{-20pt}
%     \caption{Trajectory results for $t = 0 \sim 10 (\mathrm{s})$ with end-effector axes attached are plotted.}
%     \label{fig:3d_traj}
% \end{figure}

% \subsection{Regulation}
% The desired configuration for the regulation is given by
% \begin{align}
%     p_d &= [-0.5, 0.2, 0.3]^T, \quad R_d = R_0.
% \end{align}
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/comparison_xyz.png}
%     \caption{Trajectories of end-effector in $x$, $y$, and $z$ coordinates are plotted. Red lines are for the proposed control, black dotted lines are for the benchmark control.}
%     \label{fig:regulation_comparison_xyz}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width =0.9\columnwidth]{figures/geo_3d.png}
%     \caption{Trajectory with the frame of end-effector of the proposed control in 3d plot. Red lines are $x$ axis, blue lines are $y$ axis, and green lines are $z$ axis in end-effector frame.}
%     \label{fig:regulation_geo_3d}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width =0.9\columnwidth]{figures/imp_3d.png}
%     \caption{Trajectory with the frame of end-effector of the benchmark approach in 3d plot. Red lines are $x$ axis, blue lines are $y$ axis, and green lines are $z$ axis in end-effector frame.}
%     \label{fig:regulation_imp_3d}
% \end{figure}
% The Cartesian trajectories results for the proposed control and benchmark approach is plotted in Fig.~\ref{fig:regulation_comparison_xyz}. In addition, the trajectories in 3D together with the frame for the proposed control and the conventional impedance control are plotted in Fig.~\ref{fig:regulation_geo_3d} and ~\ref{fig:regulation_imp_3d}, respectively. To compare the energy usage between two controllers, we used root-mean-squared (RMS) values of each torque inputs. The results for control inputs are summarized in the Table.~\ref{table:rms_of_inputs}. One can easily notice that the proposed control inputs uses significantly less torque inputs, while not sacrificing the control performances at all as can be shown in the Fig.~\ref{fig:regulation_comparison_xyz}.
% \begin{table}[ht]
%   \caption{RMS values of control inputs for the regulation case}
%   \label{table:rms_of_inputs}
%   \scriptsize
%   \centering%
%   \begin{tabu}[width=\columnwidth]{%
%       c| c | c
%     }
%     \toprule
%      Torque inputs & Benchmark & Proposed\\
%     \midrule
%     $T_1$ & 24.341 & 2.8613\\
%     $T_2$ & 124.85 & 53.4338\\
%     $T_3$ & 96.410 & 11.8539\\
%     $T_4$ & 86.421 & 0.6982\\
%     $T_5$ & 57.931 & 0.0844\\
%     $T_6$ & 32.093 & 3.387e-04\\
%     \bottomrule
%   \end{tabu}
% \end{table}

==> chapters/ch4_sim_old.tex <==
% We utilize the UR5e model as our robot model, which are designed using Robotic Toolbox Matlab (\cite{corke2002robotics}) in the matlab environment.
% \AR{I would suggest: We utilize the UR5e model [\cite{corke2002robotics}] implemented in matlab [version; cite matlab].}
We utilize the UR5e robot model implemented in Matlab~R2021a using \cite{corke2002robotics}. %(version R2021a).
%
As a benchmark, we use conventional impedance control implemented in \cite{robosuite2020, ochoa2021impedance}.
%
The simulation is conducted for an aggressive trajectory tracking scenario. 
%
We set the same desired impedance to both  controllers, starting from the same initial conditions,  and then we compare their performances in terms of tracking.
%
The initial conditions in all cases are
\begin{equation}\begin{aligned}
    q &= [0,0,0,0,0,0]^T, \quad \dot{q} = [0,0,0,0,0,0]^T
\end{aligned}\end{equation}
Desired impedance are set as
\begin{equation}\begin{aligned}
    K_g = \text{diag}\left([k_p,k_p,k_p,k_o,k_o,k_o]\right), \quad K_d = k_d I
    %K_d &= \text{diag}([k_d,k_d,k_d,k_d,k_d,k_d])
\end{aligned}\end{equation}
where $k_p\!=\!k_o\!=\!100$ and $k_d\!=\!50$. 
The desired trajectories are selected as 
\begin{align}
    p_d(t) &= \begin{bmatrix}-0.5\!+\!0.20 \cos{t} & 0.20\sin{t} & 0.2 \!+\! 0.05\sin{(0.8t)}\end{bmatrix}^T \nonumber\\
    R_d(t) &= R_0 
\end{align}
The resulting trajectories are plotted in Fig.~\ref{fig:comparison_xyz}. 
%
When the trajectories are aggressive, it can be noticed  that the  control strategy proposed in this paper clearly outperforms the benchmark approach  since the proposed controller properly accounts for errors in the $\SE$ structure.
%
\begin{figure}[b!]
    %\centering
    %\includegraphics[width=\columnwidth]{figures/comparison_xyz.eps}
    \vspace{-5pt}
    \hspace{-8pt}
    \input{figures/comparison_xyz.tex}
    \vspace{-20pt}
    \caption{The trajectory tracking results in $x$, $y$, and $z$ coordinates for the proposed and benchmark approach are plotted.}
    \label{fig:comparison_xyz}
\end{figure}
%
The resulting error function \eqref{eq:err_fun_SE3} are plotted in Fig.~\ref{fig:err_fun}.
%
\begin{figure}
    %\centering
    %\includegraphics[width=\columnwidth]{figures/error_func.eps}
    \vspace{-5pt}
    \hspace{-6pt}
     \input{figures/error_func.tex}
     \vspace{-20pt}
    \caption{Error function  \eqref{eq:err_fun_SE3} for the resulting trajectories.}
    \label{fig:err_fun}
\end{figure}
%
The root mean squared error values in the Cartesian coordinates are presented in Tab.~\ref{table:rms_of_errors}. 
%
\begin{table}[b!]
  \caption{RMS error values for positions}
  \label{table:rms_of_errors}
  \scriptsize
  \centering%
  \begin{tabu}[width=\columnwidth]{%
      c| c | c
    }
    \toprule
    Spatial coordinate error & Benchmark & Proposed\\
    \midrule
    $\text{RMS}(x(t) - x_d(t))$ & 0.0480 & 0.0320\\
    $\text{RMS}(y(t) - y_d(t))$ & 0.0643 & 0.0342\\
    $\text{RMS}(z(t) - z_d(t))$ & 0.0535 & 0.0182\\
    \bottomrule
  \end{tabu}
\end{table}
%
As can be shown in the results presented in Fig.~\ref{fig:comparison_xyz}, \ref{fig:err_fun}, and Tab.~\ref{table:rms_of_errors} the proposed control design outperforms the benchmark control. 
The Matlab code for the implementation of the controller proposed in this paper is provided in: \url{https://github.com/Joohwan-Seo/Geometric-Impedance-Control-Public}.\\
%
Few remarks on the actual implementation are given.
\begin{rem} 
    From the implementation perspective, the normal PD control given by
    $\tilde{T}\!=\!-K_g \eg \!-\! K_d \ev$
    can be utilized when the Jacobin matrix is numerically near singular.
    %
    This implies that even without dynamic parameters and solving inverse kinematics, we can solve the end-effector positioning problem, which has already been emphasized in an earlier work 
    \cite{hogan1985impedance}.
    %
    % This means that we may not need to solve for the inverse kinematics without any dynamic parameters, which has been already emphasized in an earlier of the work \cite{hogan1985impedance}.
% In the implementation perspective, the normal PD control given by 
%         \begin{align} \label{eq:PD_control}
%             \tilde{T} = -K_g \eg - K_d \ev 
%         \end{align}
%         can be utilized when the Jacobin matrix is numerically near singular. 
\end{rem}

\begin{figure}
    %\centering
    \vspace{-5pt}
    \hspace{-8pt}
    \input{figures/trajectory_3d.tex}
    \vspace{-20pt}
    \caption{Trajectory results for $t = 0 \sim 10 (\mathrm{s})$ with end-effector axes attached are plotted.}
    \label{fig:3d_traj}
\end{figure}

% \subsection{Regulation}
% The desired configuration for the regulation is given by
% \begin{align}
%     p_d &= [-0.5, 0.2, 0.3]^T, \quad R_d = R_0.
% \end{align}
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/comparison_xyz.png}
%     \caption{Trajectories of end-effector in $x$, $y$, and $z$ coordinates are plotted. Red lines are for the proposed control, black dotted lines are for the benchmark control.}
%     \label{fig:regulation_comparison_xyz}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width =0.9\columnwidth]{figures/geo_3d.png}
%     \caption{Trajectory with the frame of end-effector of the proposed control in 3d plot. Red lines are $x$ axis, blue lines are $y$ axis, and green lines are $z$ axis in end-effector frame.}
%     \label{fig:regulation_geo_3d}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width =0.9\columnwidth]{figures/imp_3d.png}
%     \caption{Trajectory with the frame of end-effector of the benchmark approach in 3d plot. Red lines are $x$ axis, blue lines are $y$ axis, and green lines are $z$ axis in end-effector frame.}
%     \label{fig:regulation_imp_3d}
% \end{figure}
% The Cartesian trajectories results for the proposed control and benchmark approach is plotted in Fig.~\ref{fig:regulation_comparison_xyz}. In addition, the trajectories in 3D together with the frame for the proposed control and the conventional impedance control are plotted in Fig.~\ref{fig:regulation_geo_3d} and ~\ref{fig:regulation_imp_3d}, respectively. To compare the energy usage between two controllers, we used root-mean-squared (RMS) values of each torque inputs. The results for control inputs are summarized in the Table.~\ref{table:rms_of_inputs}. One can easily notice that the proposed control inputs uses significantly less torque inputs, while not sacrificing the control performances at all as can be shown in the Fig.~\ref{fig:regulation_comparison_xyz}.
% \begin{table}[ht]
%   \caption{RMS values of control inputs for the regulation case}
%   \label{table:rms_of_inputs}
%   \scriptsize
%   \centering%
%   \begin{tabu}[width=\columnwidth]{%
%       c| c | c
%     }
%     \toprule
%      Torque inputs & Benchmark & Proposed\\
%     \midrule
%     $T_1$ & 24.341 & 2.8613\\
%     $T_2$ & 124.85 & 53.4338\\
%     $T_3$ & 96.410 & 11.8539\\
%     $T_4$ & 86.421 & 0.6982\\
%     $T_5$ & 57.931 & 0.0844\\
%     $T_6$ & 32.093 & 3.387e-04\\
%     \bottomrule
%   \end{tabu}
% \end{table}

==> chapters/ch5_conclu_old.tex <==
%The
A novel impedance control law considering geometric structure of the manipulator is proposed in this paper.
%
The left-invariant error metric is first defined and the geometrically consistent error vectors are derived.
%
Based on the error vectors, the geometric impedance control rule is obtained from the dissipative property of the energy function. 
%
The stability analysis shows that the closed-loop system is asymptotically stable.
%
In simulation, %experiment, 
we showed that the proposed control outperformed the conventional control in trajectory tracking.

As a future work, we will combine the proposed geometric impedance control with reinforcement learning to solve robotic manipulation task problems.
%
% Since the controller will behave well, we expect an improvement in performance compared to state of the art methods.
%
Since the controller is now defined appropriately, we expect an improvement in performance compared to state of the art methods.
%
Above that, we will also research on the solution of robotic tasks where the tasks can be better encoded as velocity fields instead of desired trajectories, i.e., closed-loop system lying on the desired manifold.
%Based on the proposed geometric impedance control, we hope to solve robotic task problem using reinforcement learning.
%
%We conjecture that the using correct error vectors can be helpful since the controller will well-behave.
%
%Furthermore, we are also interested in robotic task problem where tasks can be better encoded as velocity field, instead of desired trajectories, i.e., closed-loop system lying on desired manifold.
